OVRseen: Auditing Network Traffic and Privacy Policies in Oculus VR

Virtual reality (VR) is an emerging technology that enables new applications but also introduces privacy risks. In this paper, we focus on Oculus VR (OVR), the leading platform in the VR space and we provide the first comprehensive analysis of personal data exposed by OVR apps and the platform itself, from a combined networking and privacy policy perspective. We experimented with the Quest 2 headset and tested the most popular VR apps available on the official Oculus and the SideQuest app stores. We developed OVRseen, a methodology and system for collecting, analyzing, and comparing network traffic and privacy policies on OVR. On the networking side, we captured and decrypted network traffic of VR apps, which was previously not possible on OVR, and we extracted data flows, defined as <app, data type, destination>. Compared to the mobile and other app ecosystems, we found OVR to be more centralized and driven by tracking and analytics, rather than by third-party advertising. We show that the data types exposed by VR apps include personally identifiable information (PII), device information that can be used for fingerprinting, and VR-specific data types. By comparing the data flows found in the network traffic with statements made in the apps' privacy policies, we found that approximately 70% of OVR data flows were not properly disclosed. Furthermore, we extracted additional context from the privacy policies, and we observed that 69% of the data flows were used for purposes unrelated to the core functionality of apps.

==> VR Project (USENIX Security 2022)/abstract.tex <==
%-------------------------------------------------------------------------------
\begin{abstract}
%-------------------------------------------------------------------------------
\begin{comment}
Virtual reality (VR) technology is a newly emerging market that
has been gaining a lot of attention in recent years.
Compared to other existing platforms (\eg mobile phones, smart TVs, \etc), we observe that the VR platform comes with new privacy risks.
More specifically, a VR device is equipped with sensors that collect data from user's physical movement, body pose, voice activity, hand tracking, facial expressions, and even play area---\emph{these potentially reveal some information about the user's physical characteristics and home!}
%A VR device typically consists of a headset and hand controllers.
%Its usage model requires users to immersively interact with the VR environment visible through the headset.
%At the same time, the VR device is equipped with sensors that collect data from user's physical movement, body pose, voice activity, hand tracking, facial expressions, and even play area---\emph{these potentially reveal some information about the user's physical characteristics and home!}
\end{comment}

Virtual reality (VR) is an emerging technology that enables new applications but also introduces privacy risks. In this paper, we focus on Oculus VR (\oculusvr{}), the leading platform in the VR space and we provide the first comprehensive analysis of personal data exposed by \oculusvr{} apps and the platform itself, 
from a combined networking and privacy policy perspective.  We experimented with the \device{} headset and tested the most popular VR apps available on the official Oculus and the Side\-Quest app stores.  We developed \tool{}, a methodology and system for collecting, analyzing, and comparing network traffic and privacy policies on \oculusvr{}. On the networking side, we captured and decrypted network traffic of VR apps, which was previously not possible on \oculusvr{}, and we extracted data flows, defined as \dataflowtuple{}. 
Compared  to the mobile and other app ecosystems, we found \oculusvr{} to be more centralized and driven by tracking and analytics, rather than by third-party advertising. 
We show that the data types exposed by VR apps include personally identifiable information (PII), device information that can be used for fingerprinting, and VR-specific data types. By comparing the data flows found in the network traffic with statements made in the apps' privacy policies, we
found that approximately 70\% of \oculusvr{} data flows were not properly disclosed. Furthermore, we extracted additional context % including the purpose, 
from the privacy policies, and we observed that 69\% of the data flows were used for purposes unrelated to the core functionality of apps.  
%\athina{[other highlights?]}

\mycomment{
We also used \tool{} to analyze privacy policies on \oculusvr{}---\tool{} integrates two state-of-the-art tools called \policheck{} and \polisys{}.
In \tool{}, \policheck{} is significantly improved---we adapted its data and entity ontologies into the VR context.
We used \tool{}'s \policheck{} to perform data-flow-to-policy consistency analysis. We discovered that approximately 70\% of data flows on \oculusvr{} are currently not properly disclosed.  
Finally, \tool{} also integrates \polisys{} to analyze privacy policies and characterize the purpose of the identified data flows.
}

\begin{comment}
In this paper, we comprehensively evaluated the privacy aspects of the VR platform.
We performed our study on the Oculus platform, a popular VR platform that the research community has recently been focusing on for VR research.
We experimented with 150 VR apps from both the official Oculus app store and a third-party app store called SideQuest. As our dataset, we collected network traffic for these apps on \device{}.
Using this dataset, we then performed a complete evaluation of data exposures and privacy policy consistency.
Among unique identifiers (\eg device ID) that have been long considered as \emph{personally identifiable information} (PII), we found that these data exposures include new VR-specific data types (\eg physical movement, play area, \etc).
On the other hand, we also discovered that many app developers did not properly disclose their data collection practices in their privacy policies.
%First, we found that the ATS ecosystem is dominated by Oculus (\ie Facebook) as first party.
%We also discovered that the platform indeed collects new VR-specific data types (\eg physical movement, play area, \etc).
%Finally, we found that many app developers did not properly disclose their data collection practices in their privacy policies.
\end{comment}

\end{abstract}

==> VR Project (USENIX Security 2022)/acknowledgment.tex <==
\minorrevision{
\section*{Acknowledgment}
\label{sect:acknowledgment}

This project was supported by NSF Awards 1815666 and 1956393.
We would like to thank our shepherd, Tara Whalen, and the USENIX Security 2022 reviewers for their feedback, which helped to significantly improve the paper. 
We would also like to thank Yiyu Qian, for his help with part of our data collection process. 
}

==> VR Project (USENIX Security 2022)/additional.tex <==
\subsection{Data Minimization}
We evaluate whether the transmission of data is necessary to the functionality of an Oculus App. For that purpose, we sample a few apps based on criteria such as if they were chatty. We also randomly sample a few apps to do the following:
\begin{itemize}
    \item Offline mode: We block all network traffic to see if they are still functional. 
    \item No platform mode: We block all network traffic going to Facebook.
    \item No X system apps: We block all network traffic initiated by certain system apps. We report which system apps are important to the functionality of apps.
    \item No network traffic from app: we block all network traffic initiated by the app itself.
\end{itemize}

==> VR Project (USENIX Security 2022)/ats_pii.tex <==
%\subsection{Network Traffic Analysis}
%\label{sec:ats-pii-analyses}
%
%To provide party context, we leverage the methodology in \secref{}~\ref{sec:labeling}, which reveals whether a packet was initiated as a first, third, or platform-party. 

\begin{comment} %%%% moved up in latex
%\myparagraph{Overview.}
\begin{figure*}[t!]
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/plots_temp/app_and_esld_third_and_platform_party_paper.pdf}
        \vspace{-2em}
        \caption{}
        \label{fig:top-esld-third-and-platform-party}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/plots_temp/app_and_fqdn_ats_third_and_platform_party_paper.pdf}
        \vspace{-2em}
        \caption{}
        \label{fig:top-ats-third-and-platform-party}
    \end{subfigure}
    \caption{Top-10 platform and third-party (a) eSLDs and (b) ATS FQDNs ordered by the number of apps that contact them.}
    \label{fig:top-esld-ats}
\end{figure*}
\end{comment}

\subsection{\oculusvr{} Advertising \& Tracking Ecosystem}
\label{sec:ats-ecosystem}
In this section, we explore the destination domains found in our network traffic dataset (see \secref{}~\ref{sec:labeling-data-flow}).
\figref{}~\ref{fig:top-esld-third-and-platform-party} presents the top-10 eSLDs for platform and third-party. 
We found that, unlike the mobile ecosystem, the presence of third-parties is minimal and platform traffic dominates in all apps (\eg{} $oculus.com$, $facebook.com$).
%As expected, Facebook dominates by being present in all apps (\eg{} $oculus.com$, $facebook.com$).
%Conversely, we found that unlike the mobile ecosystem, the presence of third-parties is minimal.
% 
The most prominent third-party organization is Unity (\eg{} \textit{unity3d.com}), which appears in 68 out of 140 apps (49\%). 
This is expected since 96 apps in our dataset were developed using the Unity engine (see \secref{}~\ref{sec:network-traffic-dataset-raw}).
Conversely, although 31 apps in our dataset were developed using the Unreal engine, it does not appear as a major third-party data collector because Unreal does not provide its own analytics service. %~\cite{unreal-analytics}.
%
Beyond Unity, other small players include Alphabet (\eg{} \textit{google.com},  \textit{cloudfunctions.net}) and Amazon (\eg{} \textit{amazonaws.com}).
%
In addition, 87 out of 140 apps contact four or fewer third-party eSLDs (62\%). 
%
%Finally, we found that 46 out of 138 apps (33\%) contact their own first-party eSLD.

\myparagraph{Identifying ATS domains.} 
To identify ATS domains, we apply the following popular domain-based blocklists:
%In \tool{}, we leverage three state-of-the-art and popular DNS-based blocklists to identify ATS domains. For the rest of the paper, when we refer to blocklists, we specifically mean:
(1) \textit{PiHole's Default List}~\cite{pihole-homepage}, a list that blocks cross-platform ATS domains for IoT devices;
(2) \textit{Mother of All Adblocking}~\cite{moab}, a list that blocks both ads and tracking domains for mobile devices; and
(3) \textit{Disconnect Me}~\cite{disconnectme}, a list that blocks tracking domains.
For the rest of the paper, we will refer to the above lists simply as ``blocklists''.
We note that there are no blocklists that are curated for VR platforms. 
Thus, we choose blocklists that balance between IoT and mobile devices, and one that specializes in tracking. 


\myparagraph{\oculusvr{} ATS ecosystem.} The majority of identified ATS domains relate to social and analytics-based purposes. \figref{}~\ref{fig:top-ats-third-and-platform-party} provides the top-10 ATS FQDNs that are labeled by our \blocklist{s}. 
We found that the prevalent platform-related FQDNs along with Unity, the prominent third party, are labeled as ATS. This is expected: domains such as \textit{graph.oculus.com} and \textit{perf-events.cloud.unity3d.com} are utilized for social features like managing leaderboards %~\cite{oculus-leaderboards} 
and app analytics, %~\cite{unity-analytics},
respectively.
We also consider the presence of organizations based on the number of unique domains contacted.
%
The most popular organization is Alphabet, which has 13 domains, such as \textit{google-analytics.com} and \textit{firebase-settings.crashlytics.com}. Four domains are associated with Facebook, such as \textit{graph.facebook.com}. Similarly, four are from Unity, such as \textit{userreporting.cloud.unity3d.com} and \textit{config.uca.cloud.unity3d.com}. 
Other domains are associated with analytics companies that focus on tracking how users interact with apps (\eg{} whether they sign up for an account) such as \textit{logs-01.loggly.com}, \textit{api.mixpanel.com}, and \textit{api2.amplitude.com}.
%
\mycomment{
The most popular organization is Alphabet, which has 13 domains, such as \textit{google-analytics}~\cite{google-analytics} and \textit{firebase-settings.crashlytics.com}~\cite{crashlytics}. Four domains are associated with Facebook, such as \textit{graph.facebook.com}~\cite{facebook-graph-api}. Similarly, four are from Unity, such as \textit{userreporting.cloud.unity3d.com} and \textit{config.uca.cloud.unity3d.com}\cite{unity-analytics}. 
Other domains are associated with analytics companies that focus on tracking how users interact with apps (\eg{} whether they sign up for an account) such as \textit{logs-01.loggly.com}~\cite{loggly}, \textit{api.mixpanel.com}~\cite{mixpanel}, and \textit{api2.amplitude.com}~\cite{amplitude-analytics}.}\minorrevision{Lastly, we provide an in-depth comparison to other ecosystems in~\secref{}~\ref{sec:major-findings}.}

% majority of content merged into 5.1
\mycomment{
\myparagraph{\oculusvr{} vs. Android and Smart TV.} When comparing the \oculusvr{} ATS ecosystem with the more mature Android~\cite{shuba2020nomoats, razaghpanah2018apps} and Smart TVs (\eg{} Roku and Amazon's FireTV)~\cite{varmarken2020tv, mohajeri2019watching}, the biggest difference is that \oculusvr{} does not have discernible ad-related domains. For example, while Roku has \textit{ads.tremorhub.com}, FireTV has \textit{amazon-adsystem.com}, and Android has \textit{doubleclick.net}, \oculusvr{} only has their tracking counterparts. 
\rahmadi{We surmise that this is because Facebook wants all ads to be within its own ad ecosystem.}
%We surmise that this is because Facebook wants all ads to be within its own ad ecosystem~\cite{facebook-ads}. 
Facebook's move to force new \oculusvr{} users to have a Facebook account in late 2020 points to this possibility~\cite{oculus-blog-force-login}. 
However, the \oculusvr{} ATS ecosystem does contain other major key-players, such as Unity and Alphabet, that are also present in the other two ecosystems. 
Still, Unity domains that are related to ads (\eg \textit{unityads.unity3d.com}~\cite{razaghpanah2018apps}) do not appear in the \oculusvr{} ATS ecosystem. 
Furthermore, the \oculusvr{} ATS ecosystem is not as diverse---it misses big companies like Amazon, Comscore, Inc (\eg{} \textit{scorecardresearch.com}) and Adobe (\eg{} \textit{dpm.demdex.net})~\cite{varmarken2020tv}. 
}

\begin{table}[t!]
	\tabletextsize
	\centering
	\begin{tabularx}{\linewidth}{p{3.9cm} p{2cm} p{1.4cm} }
	    \toprule
		\textbf{FQDN} & \textbf{Organization} & \textbf{Data Types} 
		\\
		\midrule
		bdb51.playfabapi.com & Microsoft & 11 \\
		%bdb51.playfabapi.com, 1c31b.playfabapi.com & Microsoft & Android ID, User ID, Device ID, Person Name, Email, Geolocation, Hardware Info, System Version, App Name, Session Info, VR Movement  \\
		\midrule
		sharedprod.braincloudservers.com & bitHeads Inc. & 8   \\
		%sharedprod.braincloudservers.com & bitHeads Inc. & User ID, Geolocation, Hardware Info, System Version, SDK Version, App Name, Session Info, Language  \\
		\midrule
		cloud.liveswitch.io & Frozen Mountain Software & 7 \\
		%cloud.liveswitch.io & Frozen Mountain Software & User ID, Device ID, Hardware Info,  System Version, App Name, Language, Cookie \\
		\midrule
		datarouter.ol.epicgames.com & Epic Games & 6 \\
		%datarouter.ol.epicgames.com & Epic Games & User ID, Device ID, Hardware Info, SDK version, App Name, Session Info  \\
		\midrule
		9e0j15elj5.execute-api.us-west-1.amazonaws.com & Amazon & 5  \\ 
		%9e0j15elj5.execute-api.us-west-1.amazonaws.com & Amazon & User ID, Hardware Info, System Version, SDK Version, Usage Time  \\ 
	    \bottomrule
	\end{tabularx}
	\caption{Top-5 third-party FQDNs that are missed by blocklists based on the number of data types exposed.}
	\vspace{-1em}
	\label{tab:missed-fqdns}
\end{table} 

\mycomment{
\begin{table}[t!]
	\tabletextsize
	\centering
	\begin{tabularx}{\linewidth}{p{33mm} | r r r}
	    \toprule
	    \multicolumn{1}{c|}{Data Types (21)} &  \multicolumn{3}{c}{\textsf{Destination Party }} \\
		\textbf{PII}  & \textbf{First} &  \textbf{Third} &  \textbf{Platform}  \\
		\midrule
        Android ID & 6/6/17\%  & 31/7/43\% & 18/2/50\% \\
        Device ID & 6/6/0\% & 64/13/38\% & 2/1/100\% \\
        Email  & 2/2/0\% & 5/5/20\%  & - \\
	    Geolocation & - & 5/4/50\%  & - \\
		Person Name & 1/1/0\% & 7/4/50\% & - \\
		Serial Number  & - & - & 18/2/50\%  \\
		User ID  & 5/5/20\% & 65/13/38\% & - \\

		\midrule	
		\multicolumn{4}{l}{\textbf{Fingerprint}} \\
		\midrule
        App Name  & 4/4/25\% & 65/10/40\% & 2/1/100\% \\
        Build Version  & - & 61/3/100\% & -  \\
        Cookies  & 5/5/0\% & 4/3/33\% & 2/1/100\% \\
        Flags  & 6/6/0\% & 53/8/50\% & 2/1/100\% \\
        Hardware Info  &  21/25/4\% & 65/23/39\% & 19/3/33\% \\
        SDK Version & 23/34/6\% & 69/28/46\% & 20/4/0\% \\
        Session Info  & 7/7/14\% & 66/13/46\% & 2/1/100\% \\
        System Version  & 16/20/5\% & 62/21/43\% & 19/3/33\% \\
        Usage Time & 2/2/0\% & 59/4/50\% & - \\
        Language  & 5/5/0\% & 28/9/56\% & 16/1/0\% \\
        \midrule
        \multicolumn{4}{l}{\textbf{VR Sensory Data}} \\ 
        \midrule
        VR Field of View & - & 16/1/100\% & - \\
        VR Movement  & 1/1/0\% & 24/6/67\% & 2/1/100\% \\
        VR Play Area  & - & 40/1/100\% & - \\
        VR Pupillary Distance & - & 16/1/100\% & - \\

       \midrule
       \rowcolor{brandeisblue!10}
        \textbf{Total} & 33/44/5\% & 70/39/36\% & 22/5/20\% \\
	    \bottomrule
	\end{tabularx}
		\vspace{-5pt}
	\caption{\textbf{Data Types Exposed in Our Network Traffic Dataset.} We report: ``Number of apps that send the data type to a destination by party / FQDNs that receive the data type / \% of FQDNs blocked by \blocklist{s}.'' 
	%On the right column, we provide aggregated information across both app stores. The last row provides aggregated information across all data types. Notably, they consider the data in terms of unique apps and unique FQDNs.
	}
	\vspace{-10pt}
	\label{tab:pii-summary}
\end{table}
}

\myparagraph{Missed by blocklists.} 
The three \blocklist{s} that we use in \tool{} are not tailored for the Oculus platform. As a result, there could be domains that are ATS related but not labeled as such. To that end, we explored and leveraged data flows to find potential domains that are missed by \blocklist{s}. In particular, we start from data types exposed in our network traffic, and identify the destinations where these data types are sent to.  \tabref{}~\ref{tab:missed-fqdns} summarizes third-party destinations that collect the most data types and are {\em not} already captured by any of the \blocklist{s}.
%
We found the presence of 11 different organizations, not caught by blocklists, including: Microsoft, bitHeads Inc., and Epic Games---the company that created the Unreal engine. 
%
The majority are cloud-based services that provide social features, such as messaging, and the ability to track users for engagement and monetization (\eg{} promotions to different segments of users). %~\cite{azure-business-intel, gamesparks}. 
%
We provide additional FQDNs missed by blocklists in \appdx{\appref{}~\ref{app:missed-blocklists}}.

\mycomment{
We found the presence of 11 different organizations, not caught by blocklists, including: Microsoft~\cite{microsoft-playfab}, bitHeads Inc.~\cite{bitheads}, and Epic Games (the company that created the Unreal engine)~\cite{epicgames}. The majority are cloud-based services that provide social features, such as messaging, and the ability to track users for engagement and monetization (\eg{} promotions to different segments of users)~\cite{azure-business-intel, braincloud-features, gamesparks}. We provide additional FQDNs missed by blocklists in \appref{}~\ref{app:missed-blocklists}.}

\begin{table}[t!]
	\tabletextsize
	\centering
	\minorrevision{
	\begin{tabularx}{\columnwidth}{ p{18mm} | r r r | r r r | r r r}
	%\begin{tabularx}{\linewidth}{ p{25mm} | X X X | X X X | X X X}
	    \toprule
	    %\multicolumn{1}{l|}{Data Types (21)} & 
	    %\multicolumn{3}{c|}{} & 
	    %\multicolumn{6}{c}{} \\
		\multicolumn{1}{l|}{Data Types (21)}  & \multicolumn{3}{c|}{\textbf{Apps}} &  \multicolumn{3}{c}{\textbf{FQDNs}} &  \multicolumn{3}{c}{\textbf{\% Blocked}}  \\
		%\midrule
		\multicolumn{1}{l|}{\textbf{PII}} & 
		\multicolumn{1}{X}{1\textsuperscript{st}} & 
		\multicolumn{1}{X}{3\textsuperscript{rd}} & 
		\multicolumn{1}{X|}{Pl.} & 
		\multicolumn{1}{X}{1\textsuperscript{st}} & 
		\multicolumn{1}{X}{3\textsuperscript{rd}} & 
		\multicolumn{1}{X|}{Pl.} & 
		\multicolumn{1}{X}{1\textsuperscript{st}} & 
		\multicolumn{1}{X}{3\textsuperscript{rd}} & 
		\multicolumn{1}{X}{Pl.} 
		\\
        
		\midrule
        Device ID  & 6 & 64 & 2  & 6 & 13 & 1 & 0 & 38 & 100 \\
		User ID  & 5 & 65 & 0 & 5 & 13 & 0 & 20 & 38 & - \\
        Android ID & 6 & 31 & 18 & 6 & 7  & 2 & 17 & 43 & 50 \\
		Serial Number & 0 & 0 & 18 & 0 & 0 & 2 & - & - & 50  \\
		Person Name & 1 & 7 & 0 & 1 & 4 & 0 & 0 & 50 & - \\
        Email  & 2 & 5 & 0 & 2 & 5 & 0 & 0 & 20 & - \\
	    Geolocation & 0 & 5 & 0 & 0 & 4 & 0 & - & 50 & - \\
		\midrule	
		\multicolumn{10}{l}{\textbf{Fingerprint}} \\
		\midrule
        SDK Version & 23 & 69 & 20 & 34 & 28 & 4 & 6 & 46 & 0 \\
        Hardware Info & 21 & 65 & 19 & 25 & 23 & 3 & 4 & 39 & 33 \\
        System Version & 16 & 62 & 19 & 20 & 21 & 3 & 5 & 43 & 33 \\
        Session Info  & 7 & 66 & 2 & 7 & 13 & 1 & 14 & 46 & 100 \\
        App Name  & 4 & 65 & 2 & 4 & 10 &1 & 25 & 40 & 100 \\
        Build Version  & 0 & 61 & 0 & 0 & 3 & 0 & - & 100 & -  \\
        Flags  & 6 & 53 & 2 & 6 & 8 & 1 & 0 & 50 &100 \\
        Usage Time & 2 & 59 & 0 & 2 & 4 & 0 & 0 & 50 & - \\        
        Language  & 5 & 28 & 16 & 5 & 9 & 1 & 0 & 56 & 0 \\
        Cookies  & 5 & 4 & 2 & 5 & 3 & 1 & 0 & 33 & 100 \\
        \midrule
        \multicolumn{10}{l}{\textbf{VR Sensory Data}} \\ 
        \midrule
        VR Play Area  & 0 & 40 & 0 & 0 & 1 & 0 & - & 100 & - \\
        VR Movement  & 1 & 24 & 2 & 1 & 6 & 1 & 0 & 67 & 100 \\
        VR~Field~of~View & 0 & 16 & 0 & 0 & 1 & 0 & - & 100 & - \\
        VR Pupillary & 0 & 16 & 0 & 0 & 1 & 0 & - & 100 & - \\
        Distance & & & & & & & & & \\

       \midrule
       \rowcolor{brandeisblue!10}
        \textbf{Total} & 33 & 70 & 22 & 44 & 39 & 5 & 5 & 36 & 20 \\
	    \bottomrule
	\end{tabularx}
		\vspace{-5pt}
		}
	\caption{\textbf{Data types exposed in the network traffic dataset.}
	\minorrevision{Column ``Apps'' reports the number of apps that send the data type to a destination; column ``FQDNs'' reports the number of FQDNs that receive that data type; and column ``\% Blocked'' reports the percentage of FQDNs blocked by \blocklist{s}. Using sub-columns, we denote party categories: first (1\textsuperscript{st}), third (3\textsuperscript{rd}), and platform (Pl.) parties. 
	%The numbers are listed in the descending order of app prevalence \rahmadi{(\ie the sum of the ``Apps'' sub-columns)} per data type category.
	}
	}
	%For each data type, we looked at apps that send that data type to a remote destination and we report: the number of first (1\textsuperscript{st}), third (3\textsuperscript{rd}), and platform (Pl.) parties that received that data type; the number of FQDNs that receive that data type; and the \% of FQDNs blocked by \blocklist{s}. We order by decreasing number of third parties, \ie the Apps \athina{($3^{rd}$)} column.}}
	%\vspace{-10pt}
	\label{tab:pii-summary}
\end{table}







\subsection{Data Flows in Context}
\label{sec:pii-exposures}


The exposure of a particular data type, on its own, does not convey much information: it may be appropriate or inappropriate depending on the context~\cite{privacy-in-context}. For example, geolocation sent to the GoogleEarth VR or Wander VR app is necessary for the  functionality, while geolocation used for ATS purposes is less appropriate. The network traffic can be used to partly infer the purpose  of data flows, \eg depending on whether the destination being first-, third-, or platform-party; or an ATS.
%\footnote{This heuristic has been previously used in other network measurement studies such as \cite{varmarken2020tv} \athina{[ADD MORE]}. 
% For example, sending data to first-parties  is considered appropriate, as developers often collect data to provide personalized experiences or to fine-tune their apps, while data exposed to third-parties are considered  more worrisome. % as the developer does not have control over the usage of the collected data.} 
\tabref{}~\ref{tab:pii-summary} lists all data types found in our network traffic, extracted using the methods explained in \secref{}~\ref{sec:labeling-data-flow}. 
%and also characterizes the destination they are sent to: whether it is a first, third or platform party, and whether it is blocked by ATS blocklists. 
%\tabref{}~\ref{tab:pii-summary} presents the data types for both app stores.
%; a breakdown between Oculus and SideQuest app stores is provided  in~\appref{}~\ref{app:data=types}. 

%We adopt the approach from ~\cite{varmarken2020tv} to label whether an exposure is ``good'' or ``bad'' by relying on the party categorization of the destination.  If the exposure goes to a first-party entity (\ie{} developers), we consider it to be ``good,'' as developers often collect data to provide personalized experiences or to fine-tune their apps (\eg{} frame-rate, difficulty level, \etc).  On the other hand, data exposures to third-parties are considered as ``bad'' as the developer does not have control over the usage of the collected data.

\myparagraph{Third party.} 
Half of the apps (70 out of \appstotal) expose data flows to third-party FQDNs, 36\% of which are labeled as ATS by blocklists.
Third parties collect a number of PII data types, including Device ID (64 apps), User ID (65 apps), and Android ID (31 apps), indicating cross-app tracking.
In addition, third parties collect system, hardware, and version info from over 60 apps---denoting the possibility that the data types are utilized to fingerprint users.
Further, all VR specific data types, with the exception of VR Movement, are collected by a single third-party ATS domain belonging to Unity.
VR Movement is collected by a diverse set of third-party destinations, such as \textit{google-analytics.com}, \textit{playfabapi.com} and \textit{logs-01.loggly.com}, implying that trackers are becoming interested in collecting VR analytics. 
%Overall, although the blocklists did not cover some edge cases, \eg exposures to \textit{analytics.ndreams.net} (first-party game studio~\cite{nDreams}) and \textit{1c31b.playfabapi.com} (Microsoft~\cite{microsoft-playfab}), the \blocklist{s} successfully capture 71\% of these exposures. 


\myparagraph{Platform party.} 
Our findings on exposures to platform-party domains are a lower bound since not all platform traffic could be decrypted (see \secref{}~\ref{sec:limitation-conclusion}). 
However, even with limited decryption, we see a number of exposures whose destinations are five third-party FQDNs. 
Although only one of these FQDNs is labeled as ATS by the blocklists, other platform-party FQDNs could be ATS domains that are missed by blocklists (see \secref{}~\ref{sec:ats-ecosystem}). 
For example, \textit{graph.facebook.com} is an ATS FQDN, and \textit{graph.oculus.com} appears to be its counterpart for \oculusvr{}; it collects six different data types in our dataset. %~\cite{oculus-graph}.
Notably, the platform party is the sole party responsible for collecting a sensitive hardware ID that cannot be reset by the user---the Serial Number.
In contrast to OVR, the Android developer guide strongly discourages its use~\cite{android-dev-practice}.

%\myparagraph{First-party \vs{} Third-party.}
%The column ``Both App Stores'' in \tabref{}~\ref{tab:pii-summary} summarizes the exposures and block rates for all apps in our corpus.
%The majority of apps (83 apps) expose data to third-party destinations and the \blocklist{s} capture 34\% of those exposures. 
\myparagraph{First party.} 
Only 33 apps expose data flows to first-party FQDNs, and only 5\% of them are labeled as ATS.
Interestingly, the blocklists tend to have higher block rates for first-party FQDNs if they collect certain data types, \eg Android ID (17\%), User ID (20\%), and App Name (25\%).
%the block percentage is low (5\%) for data types going to first-party destinations (33 apps), with Android ID (17\%), User ID (20\%), and App Name (25\%) having the highest block rates. 
Popular data types collected by first-party destinations are Hardware Info (21 apps), SDK Version (23 apps), and System Version (16 apps). For developers, this information can be used to prioritize bug fixes or improvements that would impact the most users. Thus, it makes sense that only \textasciitilde5\% of first-party FQDNs that collect this information are labeled as ATS.
%\vspace{-10pt}
%However, the same data types are also the top-3 sent to third-parties---denoting the possibility that the data types are utilized to fingerprint users.

%The majority of VR specific data types are sent to the third-party ATS domain \textit{cdp.cloud.unity3d.com}.
%and are blocked. 
%Overall, although the blocklists did not cover some edge cases, \eg exposures to \textit{analytics.ndreams.net} (first-party game studio~\cite{nDreams}) and \textit{1c31b.playfabapi.com} (Microsoft~\cite{microsoft-playfab}), the \blocklist{s} successfully capture 71\% of these exposures. 
%The high block rate indicates that users will be protected against these exposures if the \blocklist{s} are employed.

%When comparing distinct first-party and third-party FQDNs, we found the same number of FQDNs (44) going to the respective parties. This spotlights two things within the Oculus ecosystem: (1) it indicates the effort app developers have put in improving the VR experience for users; and (2) it shows the developing nature of the ATS ecosystem. Notably, we find several data types that have low block rates for third-parties such as Android ID, Device ID, User ID, and Hardware Info all fall below 50\%. 

%%
%We compare the data type exposures for apps within the Oculus store and SideQuest. The blocklists capture more first-party exposures for SideQuest apps; particularly Android ID (20\% for SideQuest vs{} 0\% for Oculus) and Session Info (33\% for SideQuest vs{} 0\% for Oculus).
%Furthermore, SideQuest exposes Android ID to twice as many third-party FQDNs (8 FQDNs) compared the Oculus store (4 FQDNs) with block rates (38\% \vs{} 75\%). The opposite is true for Device ID. Lastly, the blocklists miss all third-party FQDNs that receive Email for SideQuest, which is mainly sent to \textit{*.playfab.com}.


\begin{comment}
    \subsubsection{System Apps.}
    \begin{figure}[ht!]
    	\centering
    	\includegraphics[width=1\columnwidth]{images/plots_temp/system-apps-vs-fqdns_heatmap_paper.pdf}
    	\caption{System Apps vs. FQDNs. \todo{will remove, visible right now for writing only}}
    	\label{fig:system-apps-fqdns}
    \end{figure}
    Recall that we cannot decrypt network traffic for system apps within the Quest2. As a result, we do not report any data type exposures for platform-party. However, to partially handle this limitation, we study the documentation on \oculusvr{} system apps, which allows us to infer the possible data types that can be sent.
\end{comment}

%Furthermore, since we cannot decrypt the majority of network traffic made by system apps, we cannot analyze exposures made by them.
 
%\subsection{Summary} \label{sec:ats-pii-summary}
\myparagraph{Summary.}
The \oculusvr{} ATS ecosystem is young when compared to Android and Smart TVs. It is dominated by tracking domains for social features and analytics, but not by ads. We have detailed 21 different data types that \oculusvr{} sends to first-, third-, and platform-parties. State-of-the-art blocklists only captured 36\% of exposures to third parties, missing some sensitive exposures such as Email, User ID, and Device ID.
%\vspace{-5pt}

%{\hieu{Add transition about looking at privacy policy next and how it has only recently been applied to mobile platforms.}}

\mycomment{
We explore a large set of data types and their exposures to first and third-parties. Blocklists capture the majority of VR Sensory exposures except for VR Movement.  The majority of apps exposure data types to third-parties and \blocklist{s} are only able to stop 32\% of the exposures. We utilize our data type findings to identify domains that are completely missed by \blocklist{s} and find ATS domains from organizations such as Microsoft and Epic Games.

Next, we explore whether these data type exposures are clearly disclosed within the app privacy policy. }


\begin{comment}
    \subsubsection{Notes}
    {\ashuba 
    \begin{itemize}
        \item Who are the key players in the ATS ecosystem in Oculus? (Show evidence that it's mostly FB and Unity)
        \item Does the ATS ecosystem look different from mobile? (Yes, it's monopolized)
        \item What about third-parties that are multi-purposed? Are they different from mobile? Who dominates here? (EasyList + EasyPrivacy may help here)
        \item What kind of PII is being collected by first and third parties? Any difference from mobile? Can we say that these are "leaks" without looking into their policies? (probably not --> motivates next section)
    \end{itemize}
    }
\end{comment}



==> VR Project (USENIX Security 2022)/background.tex <==


\section{ Oculus VR Platform and Apps}
\label{sec:background}

\mycomment{
In this section, we first provide the background on \oculusvr{} (\secref{}~\ref{sec:platform-motivation}). Further, we also discuss how data collection and privacy policy practices evolve on \oculusvr{}---this motivates our study on the privacy of VR platform (\secref{}~\ref{sec:oculusdataprivacy}).

\subsection{\oculusvr{} Platform}
\label{sec:platform-motivation}
}
%In this section, we provide the background on \oculusvr{}.

%\myparagraph{Background on OVR.} 
In this paper, we focus on the Oculus VR (\oculusvr{}), a representative of state-of-the art VR platform. A pioneer and leader in the VR space, \oculusvr{} was bought by Facebook in 2014~\cite{oculus-acquisition} (we refer to both as ``platform-party''), and it maintains to be the most popular VR platform today.  
%\oculusvr{} and Facebook (we refer to both as ``platform-party'') servers have different contexts and purposes (\eg 3D game apps \vs{} social analytics), but they seem to work seamlessly after the acquisition.
Facebook has integrated more social features and analytics to \oculusvr{} and now even requires users to sign in using a Facebook account~\cite{oculus-blog-force-login}.
%For instance, most recently \oculusvr{} users are required to sign in using a Facebook account.

We used the latest Oculus device, \device{}, for testing. 
%An estimated five million \device{} headsets were sold in six months since October 2020 alone \cite{oculus-acquisition,fb-q1-2021-earnings, oculus2-popular, oculus2-sales}.
\device{} is completely wireless: it can operate standalone and run apps, without being connected to other devices. In contrast, \eg Sony Playstation VR needs to be connected to a Playstation 4 as its game controller.
\device{} runs Oculus OS, a variant of Android 10 that has been modified and optimized to run VR environments and apps.
%
The device comes with a few pre-installed apps, such as the Oculus browser. 
VR apps are usually developed using two popular game engines called Unity~\cite{unity-framework} and Unreal~\cite{unreal-framework}. 
%\footnote{There is only a small portion of apps that use other frameworks, typically when they do not need 3D environment to operate, \eg we found a \device{} ESPN app, developed in Kotlin and used to display sports news and videos.}
%
Unlike traditional Android apps that run on Android JVM, these 3D app development frameworks compile VR apps into optimized (\ie stripped) binaries to run on \device{}~\cite{Unity-strip}.

%\myparagraph{OVR App Ecosystem.} 
Oculus has an official app store and a number of third-party app stores.
%
The Oculus app store offers a wide range of apps (many of them are paid), which are carefully curated and tested (\eg for VR motion sickness). %\footnote{To install an app from the Oculus app store, a user can search for the desired app through the app store browser on \device{} (or using the Oculus companion app on mobile phone) and install the app.} 
%
In addition to the Oculus app store, we focus on SideQuest---the most popular third-party app store endorsed by Facebook~\cite{oculus-sidequest}.
%
In contrast to apps from the official store, apps available on SideQuest are typically at their early development stage and thus are mostly free. %\footnote{To install an app from SideQuest, a user can browse and search for apps using SideQuest companion app that runs on a PC or laptop connected to a \device{} device~\cite{oculus-sidequest-installation}. The companion app uses the Android Debug Bridge (ADB) to install the app on the \device{} device.} 
Many of them transition from SideQuest to the Oculus app store once they mature and become paid apps.
%
%when they mature and become ready for official release, many of them are transitioned from SideQuest to the official Oculus app store and they become paid apps. 
%
As of March 2021, the official Oculus app store has 267 apps (79 free and 183 paid), and
%All of these apps are available on the Oculus store browser both on \device{} and its companion mobile app (see \secref~\ref{sec:platform-motivation}).
the SideQuest app store has 1,075 apps (859 free and 218 paid).


\myparagraph{Motivation: privacy risks in \oculusvr{}.} VR introduces privacy risks, some of which are similar to other Internet-based platforms \minorrevision{(\eg Android}~\cite{androidappstudy,taintdroid}, IoT devices~\cite{iotsok,iotsecurity}, Smart TVs~\cite{mohajeri2019watching,varmarken2020tv}), \etc),   
%In addition, VR has its own unique characteristics: oalso has access to sensitive user data and it has its own unique characteristics as a platform.
while others are unique to the VR platform. For example, VR headsets and hand controllers %to interact with the virtual environment visible through the headset.
%The headset and controllers 
 are equipped with sensors that collect data about the user's physical movement, body characteristics, voice activity, hand tracking, eye tracking, facial expressions, and play area~\cite{oculus-privacy-1,oculus-privacy-2,oculus-privacy-3}, which may in turn reveal sensitive  information about our physique, emotions, and home.  
\device{} can also act as a fitness tracker, thanks to the built-in Oculus Move app that tracks time spent for actively moving and amount of calories burned across all apps~\cite{oculus-move}.
\mycomment{\device{} can also act as a fitness tracker, thanks to the built-in Oculus Move app that tracks time spent for actively moving and amount of calories burned across all apps~\cite{forbes-fitness,oculus-move}.}
 %Since this usage model does not exist on other platforms, the privacy aspects of the collection of these new data types have not been widely studied by the research community.
 Furthermore, Oculus has been continuously updating their privacy policy with a trend of increasingly collecting more data over the years. Most notably, we observed a major update in May 2018, coinciding with the GDPR implementation date.
Many apps have no privacy policy, or fail to properly include the privacy policies of third-party libraries. Please see \appdx{\appref{}~\ref{sec:oculusdataprivacy}} for more detail on observations that motivated our study, and \secref{}~\ref{sec:related-work} on related work. The privacy risks on the relatively new VR platform are not yet well understood. 

%%%%%%%%%%%%%




\myparagraph{Goal and approach: privacy analysis of \oculusvr.} In this paper, we seek to characterize the privacy risks introduced when potentially-sensitive data available on the device are sent by the VR apps and/or the platform to remote destinations for various purposes. We followed an experimental and data-driven approach, and we chose to test and analyze the most popular VR apps.
%, described in the next paragraph, from two complementary points of view.  
In \secref~\ref{sec:network-traffic-analysis}, we characterize the actual behavior exhibited in the network traffic generated by these VR apps and platform. In \secref~\ref{sec:privacy-policy}, we present how we downloaded the privacy policies of the selected VR apps, the platform, and relevant third-party libraries, used NLP to extract and analyze the statements made about data collection, analyzed their consistency when compared against the actual data flows found in traffic, and extracted the purpose of data collection.


\myparagraph{App corpus.}
We selected \oculusvr{} apps that are widely used by players. 
Our app corpus consists of \minorrevision{150} popular paid and free apps from both the official Oculus app store and SideQuest. In contrast,  previous work typically considered only free apps from the official app store~\cite{androidappstudy,taintdroid,mohajeri2019watching,varmarken2020tv}.
% 
We used the number of ratings/reviews as the popularity metric, and considered only apps that received at least 3.5 stars. We selected \minorrevision{three groups of 50 apps each: (1) the top-50  free apps and (2) the top-50 paid apps from the Oculus app store, and (3) the top-50 apps from the SideQuest store.  We selected an equal number of paid and free apps from the Oculus app store to gain insight into both groups equally.} We purposely did not just pick the top-100 apps, because paid apps tend to receive more reviews from users and this would bias our findings towards paid apps. Specifically, this would make our corpus consist of 90\% paid and 10\% free apps.

Our app corpus is representative of both app stores.
Our top-50 free and top-50 paid Oculus apps constitute close to 40\% of all apps on the Oculus app store, whereas the total number of downloads of our top-50 SideQuest apps is approximately 45\% of all downloads for the SideQuest store.
%Our app corpus consists of apps from the official Oculus app store constitutes 38\% of all Oculus apps, and 45\% of all downloads from the SideQuest store.
%In our selection of SideQuest apps, we did not differentiate free and paid apps, since most SideQuest apps are free. We did not consider SideQuest apps below the top-50, because they have small user base. %:  even in our selected top 50 Sidequest apps, we found 16 apps in trial or beta versions with less than 200 ratings/reviews.
%
\minorrevision{Out of these 150 apps, selected for their popularity and representativeness, we were able to decrypt and analyze the network traffic for 140 of them for reasons explained in Section \ref{sec:network-traffic-dataset-raw}.}



\mycomment{
The store provides a companion app that runs on a PC or laptop. Users can use this companion app to install VR apps on \device{}~\cite{oculus-sidequest-installation}.
A developer that starts developing a new app often publishes the app's trial or beta version on SideQuest. Many of these apps are available on SideQuest for free---the purpose might be to attract users to try these newly developed apps. 
When an app has become more mature, its developer sometimes provides a purchase or donation link that leads to a third-party website, \eg \emph{itch.io}, \emph{Patreon.com}, \etc. After making a purchase or donation for the app, the download link for the app will be provided. Clicking on the download link will trigger the SideQuest app to invoke \code{adb} command that installs the app on the connected \device{} (see \secref{}~\ref{platform-motivation}).
When the apps are finally released, their developers will move them to the official Oculus app store.}

\mycomment{
\begin{figure}[!htb]
	\centering
	\includegraphics[width=1\linewidth]{images/longitudinal_data_types_paper.pdf}
	\caption{\textbf{Data Types for Oculus Privacy Policy} Over a span of 9 years, we show the number of data types that are identified and disclosed by the Oculus Privacy Policy from June 2012 to May 2021.}
	\label{fig:data-collection-trend}
\end{figure}
}

\mycomment{
\subsection{Data Privacy on \oculusvr{}}
\label{sec:oculusdataprivacy}

In our preliminary observation, we discovered two findings that motivate us to further study VR privacy in the context of Oculus platform.

First, we discovered that Oculus has been actively updating their privacy policy over the years.
We collected different versions of Oculus privacy policy~\cite{oculus-privacy-policy} over time using Wayback Machine~\cite{wayback-machine} and examined them manually.
Most notably, we observed a major change in their privacy policy around May 2018. We suspect that this is due to the implementation of the GDPR on May 25, 2018~\cite{gdpr-implementation}---this has required Oculus to be more transparent about its data collection practices.
For example, the privacy policy version before May 2018 declares that Oculus collects information about ``physical movements and dimensions''. 
The version after May 2018 adds ``play area'' as an example for ``physical movements and dimensions''.
Although it has not been strictly categorized as PII, ``play area'' might represent the area of one's home---it loosely contains ``information identifying personally owned property'' that can potentially be linked to an individual~\cite{pii-nist-report}.
This motivates us to empirically study the data collection practices on Oculus as a VR platform. We report how we use \tool{} to collect network traffic and study data exposures on Oculus in \secref{}~\ref{sec:network-traffic-analysis}.

Second, we found that many apps do not have privacy policies.
Even if they have one, we found that many developers neglect updating their privacy policies regularly---many of these privacy policies even do not have \emph{last updated times} information. 
We found that only around 40 (out of 267) apps from the official Oculus app store and 60 (out of 1075) apps from the SideQuest app store have updated their privacy policy texts in 2021.
Thus, we suspect that an app's actual data collection practices might not always be consistent with the app's privacy policy.
This motivates us to study how consistent an app's privacy policy describes the app's actual data collection practices.
We report how we use \tool{} to analyze privacy policies in \secref{}~\ref{sec:privacy-policy}.
}

\mycomment{
\subsection{Data Privacy on Oculus}
\label{sec:oculusdataprivacy}

In our preliminary observation, we discovered three findings that motivate us to further study VR privacy in the context of Oculus platform.

First, we discovered that the Oculus privacy policy declares the collection of VR-specific data types: ``Physical Features'' (\eg estimated hand size) and ``Environmental, Dimensions, and Movement Data'' (\eg play area and hand movement)~\cite{oculus-privacy-policy}.
Although these have not been strictly categorized as PII, they loosely contain ``personal characteristics'' and ``information identifying personally owned property'' that can potentially be linked to an individual~\cite{pii-nist-report}.

Second, we discovered that Oculus has been actively updating their privacy policy with a trend that they collect increasingly more data over the years.
\mycomment{
Unfortunately, while the platform privacy policy has become clearer and more transparent about its data collection practices, many app developers neglect their responsibility to declare their data collection practices appropriately.}
%\myparagraph{Data Collection Practices.}
We collected different versions of Oculus privacy policy~\cite{oculus-privacy-policy} over time using Wayback Machine~\cite{wayback-machine}.
This allows us to observe how the Oculus data privacy and collection practices have been changing over time.
We used PoliCheck~\cite{andow2020actions} (with the similar setup described in \secref{}~\ref{sec:privacy-policy}) to analyze the different versions of Oculus privacy policy and extract data types collected by Oculus. Next, we observed how the numbers and types of collected data change over time.

\figref{}~\ref{fig:data-collection-trend} shows a trend that in its privacy policy, Oculus increasingly declares more numbers and types of collected data over the years.
Most notably, there was a major change in numbers of collected data around May 2018. We suspect that this is due to the implementation of the GDPR on May 25, 2018~\cite{gdpr-implementation}---this has required Oculus to be more transparent about its data collection practices.
For example, the privacy policy version before May 2018 declares that Oculus collects information about ``physical movements and dimensions''. The version after May 2018 adds ``play area'' as an example for ``physical movements and dimensions''.
This motivates us to further study the data collection practices on Oculus as a VR platform---we report our findings on data exposures on Oculus in \secref{}~\ref{sec:ats-pii-analyses}.

\mycomment{
\begin{figure}[!htb]
	\centering
	\includegraphics[width=1\linewidth]{images/stores_last_updated_time_plot.pdf}
	\caption{Privacy policy last updated times for apps from the official Oculus and SideQuest app stores.}
	\label{fig:last-updated-times}
\end{figure}
}

%\myparagraph{Privacy Policy of Apps.}
Third, we found that many apps do not have privacy policies.
%\footnote{As of April 2021, we discovered that 36 (out of 262) apps in the official Oculus app store and 893 (out of 1075) apps in the SideQuest app store do not have any privacy policy texts.} 
Even if they have one, we found that many developers neglect updating their privacy policies regularly---many of these privacy policies even do not have \emph{last updated times} information. 
We found that only around 40 apps from the official Oculus app store and 60 apps from the SideQuest app store have updated their privacy policy texts in 2021.
Thus, we suspect that an app's actual data collection practices might not always be consistent with the app's privacy policy.
This motivates us to study how consistent an app's privacy policy describes the app's actual data collection practices.
We report the results of our privacy policy consistency analysis in \secref{}~\ref{sec:privacy-policy}.
}


\mycomment{
{\ashuba Main question to answer here is: what does the privacy landscape look like when looking at policies alone? According to policies:
    \begin{itemize}
        \item Do policies claim minimal data sharing? (GDRP requires that data is collected only when necessary for a specific function)
        \item What kind of data do policies claim they share? Does it make sense for this type of data to be shared? Any new data types not seen in mobile?
        \item What is the most common purpose that data is being shared for?
        \item With whom is data being shared with most often? Third parties, first parties, or platform? (Policies will probably only state about first platform, which is what Policheck found and which is what we found so far as well, but in reality that's not the case)
    \end{itemize}
I would combine Sec. 3.3 and 3.4
}
}


==> VR Project (USENIX Security 2022)/conclusion.tex <==
\minorrevision{
\section{Conclusion}
\label{sec:limitation-conclusion}
}

\minorrevision{
\paragraph{Summary.}
We present the first comprehensive study of privacy aspects for Oculus VR (\oculusvr{}), the most popular VR platform. 
%
We developed \tool{}, a methodology and system to characterize the data collection and sharing practices of the \oculusvr{} ecosystem by (1) capturing and analyzing data flows found in the network traffic of 140 popular \oculusvr{} apps, and (2) providing additional contexts via privacy policy analysis that checks for consistency and identifies the purpose of data collection.
%
\minorrevision{We make \tool{}'s implementation and datasets publicly available at \cite{ovrseen-release}.}} \inusenixversion{An extended version of this paper, including appendices, can be found in~\cite{trimananda2021auditing}.}\inarxivversion{This is the extended version of our paper, with the same title, published at USENIX Security Symposium 2022. Please take a look at our project page for more information~\cite{ovrseen-release}.}


\myparagraph{Limitations and future directions.}  
On the networking side, we were able to decrypt, for the first time, traffic of \oculusvr{} apps, but the \oculusvr{} platform itself is closed  and we could not decrypt most of its traffic. In future work, we will explore the possibility of addressing this limitation by further exploring binary analysis. 
On the privacy policy side, \policheck{} and \polisys{} rely on different underlying NLP model, with inherent limitations and incompatibilities---this motivates future work on a unified privacy policy and context analyzer.

%We experimented with 150 VR apps from both the official Oculus app store, and a third-party app store, SideQuest.
%We found that \oculusvr{} is dominated by tracking services such as Unity, Microsft, and Google. 



\mycomment{
\myparagraph{Summary.}
In this paper, we present the first comprehensive study of privacy aspects for Oculus VR (\oculusvr{}), the most popular VR platform. 
%
We developed \tool{}, a methodology and system to characterize the data collection and sharing practices of the \oculusvr{} ecosystem by (1) capturing and analyzing data flows found in the network traffic of 140 popular \oculusvr{} apps, and (2) providing additional contexts via privacy policy analysis that checks for consistency and identifies the purpose of data collection.

We identified 21 data types exposed, including PII, device information that can be utilized for fingerprinting, and VR-specific data types that have not been studied before. We found that most data types are collected by third-party entities known for tracking, social, and analytics services. 
Compared to Android and Smart TV platforms, we found that \oculusvr{} has a less diverse set of tracking services and lacks ad-related ones; state-of-the-art blocklists could block only 36\% of these third-party destinations.
%%
By analyzing the privacy policies, we found that (1) 70\% of data flows in our dataset had inconsistent disclosures, and (2) the main purposes for data collection were advertising and analytics---these corroborate our network analysis results.

%We recommend that Oculus is made open for researchers, especially to audit platform network traffic.
We also found that 27\% (38/140) apps did not provide privacy policies, 59\% (82/140) made inconsistent (omitted, incorrect, or ambiguous) disclosures, and more than 90\% (more than 130/140) did not require user consent. Furthermore, if app developers included links to the privacy policies of third-party libraries they use, the consistency of data flows would improve significantly---our results show that the consistency increased from 32\% (359/1,135) to 74\% (841/1,135) just by including Unity and Oculus privacy policies. 
%Apps should also explicitly ask users to read and consent to their privacy policy; 
%{\todo{\hieu{Facebook opening up Oculus for researchers to audit platform network traffic, developers add third- and platform-party privacy links. research tools should consider/analyze to multiple privacy policies per app.}}}

\myparagraph{Releases.} We plan to release the network traffic dataset from the top-150 apps (the first of its kind available for VR), % \packettotal{} packets,
as well as the privacy policies of VR apps and their relevant third parties. 
We will also open-source the \tool{} software, including the processing of network traffic to extract data flows, the decryption technique for Unity and Unreal, the Android-10 version of AntMonitor, and the results from privacy policy consistency checking and purpose extraction.
\todo{We should include the link here---perhaps to our group's website.}
%We plan to open-source the \tool{} code, \athina{including the novel decryption technique for unity and unreal, and the VR-specific consistency checking}. We will also make two datasets available to the research community: (1) \netdataset{} with \packettotal{} packets, (2) the \dataset{} that contains \dataflowtotal{} data flows.

\myparagraph{Limitations and Future Directions.}  On the networking side, we were able to decrypt, for the first time, traffic of \oculusvr{} apps, but the \oculusvr{} platform itself is closed  and we could not decrypt most of its traffic. In future work, we will explore the possibility of addressing this limitation by further exploring binary analysis, as well as the companion mobile app for \oculusvr{}. %, study built-in apps (\eg Oculus Move), and third-party app stores beyond SideQuest. 
On the privacy policy side, \policheck{} and \polisys{} rely on different underlying NLP models, with inherent limitations and incompatibilities---this motivates future work on a unified privacy policy and context analyzer.
%although we were able to improve several weaknesses of \policheck{}, there were inherent limitations of the NLP model and of the algorithm used, which cannot be fixed  without altering its core functionality. Based on this experience, we plan to build a policy analyzer from scratch, for integrating the extraction of collection statements, purposes, and other context.
}

\begin{comment}

We then assessed the platform through:
(1) ATS and PII, and
(2) privacy policy analyses.
We found that tracking is dominated by Oculus (\ie Facebook).
We also discovered that the platform sends new VR-specific data types.
Finally, we found that many app developers did not properly disclose their data collection practices in their privacy policies.
\end{comment}


==> VR Project (USENIX Security 2022)/data_collection.tex <==
\section{\tool{}: Network Traffic}
\label{sec:network-traffic-analysis}

In this section, we detail our methodology for collecting and analyzing network traffic. %and we analyze the network traffic they generate for data flows.
%In this section, we exercise the selected 150 apps, and we analyze the network traffic they generate for data flows.  %describe the networking side of \tool{}.
\minorrevision{
In \secref~\ref{sec:network-traffic-collection}, we present \tool{}'s system for collecting network traffic and highlight our decryption technique.}
%
Next, in \secref~\ref{sec:network-traffic-dataset}, we describe our network traffic dataset and the extracted data flows.
%First, we present an overview of its key players by identifying organizations using Crunchbase~\cite{crunchbase-homepage}. 
%
In \secref{}~\ref{sec:ats-ecosystem}, we report our findings on the \oculusvr{} ATS ecosystem by identifying domains that were labeled as ATS by popular blocklists. 
%We provide a comparative analysis to Android and SmartTV ATS ecosystems. 
%
Finally, in \secref{}~\ref{sec:pii-exposures}, we discuss data types exposures in the extracted data flows according to the context based on whether their destination is an ATS or not.

\subsection{Network Traffic Collection}
\label{sec:network-traffic-collection}
% no root for Quest --> challenges?
% traffic collection, decryption, challenges?
In this section, we present \tool{}'s system for collecting and decrypting the network traffic that apps generate (\circled{\textbf{1}} in \figref{}~\ref{fig:our-work}). 
It is important to mention that \tool{} does not require rooting \device{}, and as of June 2021, there are no known methods for doing so~\cite{failedjailbreak}.
Since the Oculus OS is based on Android, we enhanced AntMonitor~\cite{shuba2016antmonitor} to support the Oculus OS.
%we use an enhanced version of the open-source VPN-based AntMonitor~\cite{shuba2016antmonitor} tool for network traffic collection, which we had to improve to support Android 10. 
Furthermore, to decrypt TLS traffic, we use 
Frida~\cite{frida-tool}, a dynamic instrumentation toolkit. %, to bypass certificate validation.
\minorrevision{
 Using Frida to bypass certificate validation specifically for \device{} apps presents new technical challenges, compared to Android apps that have a different structure.
Next, we describe these challenges and how we address them.
}
%Test: in \S{}~\ref{sec:network-traffic-dataset}, we blah

\myparagraph{Traffic collection.}
For collecting network traffic, \tool{} integrates AntMonitor~\cite{shuba2016antmonitor}---a VPN-based tool for Android that does not require root access. It runs completely on the device without the need to re-route traffic to a server.
AntMonitor stores the collected traffic in PCAPNG format, where each packet is annotated (in the form of a PCAPNG comment) with the name of the corresponding app. 
To decrypt TLS connections, AntMonitor installs a user CA certificate. 
%For cases where decryption is not possible (\eg due to certificate pinning), AntMonitor remembers the destination domain and the app contacting it and does not attempt to decrypt the same domain-app combination in future connections.
However, since Oculus OS is a modified version of Android 10, and AntMonitor only supports up to Android 7, we made multiple compatibility changes to support Oculus OS.
In addition, we enhanced the way AntMonitor stores decrypted packets: we adjust the sequence and ack numbers to make packet re-assembly by common tools (\eg \tshark) feasible in post-processing.
%We will open-source the code so that other researchers can make use of AntMonitor, not only on \device{}, but also on other newer Android devices. 
We will submit a pull request to AntMonitor's open-source repository, so that other researchers can make use of it, not only on \device{}, but also on other newer Android devices. 
For further details, see \appdx{\appref{}~\ref{app:antmonitor-improvement}}.

%In order to enable other researchers to continue using AntMonitor in newer Android versions, we will submit a pull request to its open source repository.

\myparagraph{TLS decryption.}
Newer Android devices, such as \device{}, pose a challenge for TLS decryption: as of Android 7, apps that target API level 24 (Android 7.0) and above no longer trust user-added certificates \cite{android7tls}.
Since \device{} cannot be rooted, we cannot install AntMonitor's certificate as a system certificate.
Thus, to circumvent the mistrust of AntMonitor's certificate, \tool{} uses Frida (see \figref{}~\ref{fig:our-work}) to intercept certificate validation APIs. 
%running on an Android device, and thus it can be used on \oculusvr{} as well.
To use Frida in a non-rooted environment, we extract each app and repackage it to include and start the Frida server when the app loads. 
The Frida server then listens to commands from a Frida client that is running on a PC using ADB.
%Although typically Frida requires root privileges to run, we use it without root by modifying an app to include the Frida library and load it when the app starts---the app needs to first be repackaged with the Frida library.
%The loaded Frida library contains a server that listens to commands from a Frida client which runs on a PC and communicates with the server via ADB.
Although ADB typically requires a USB connection, we run ADB over TCP to be able to use \device{} wirelessly, allowing for free-roaming testing of VR apps.

\tool{} uses the Frida client to load and inject our custom JavaScript code that intercepts various APIs used to verify CA certificates.
In general, Android and \device{} apps use three categories of libraries to validate certificates:
(1) the standard Android library,
(2) the Mbed TLS library~\cite{unity-mbedtls} provided by the Unity SDK, and
(3) the Unreal version of the OpenSSL library~\cite{unreal-openssl}.
\tool{} places Frida hooks into the certificate validation functions provided by these three libraries.
%To bypass the validation checks performed by these libraries, we hook into the following functions: (1) the functions in \code{TrustManager} and other classes in the Android SDK~\cite{trustmanager-cert-pinning}, (2) the \code{mbedtls\_x509\_crt\_verify\_with\_profile()} function in the \code{Mbed TLS} library~\cite{mbedtls-cert-pinning}, and (3) the \code{x509\_verify\_cert()} function in the \code{OpenSSL} library~\cite{openssl-cert-pinning}.
These hooks change the return value of the intercepted functions and set certain flags used to determine the validity of a certificate to ensure that AntMonitor's certificate is always trusted.
\minorrevision{
While bypassing certificate validation in the standard Android library is a widely known technique~\cite{frida-pinning-bypass}, bypassing validation in Unity and Unreal SDKs is not. Thus, we developed the following technique.
}

%The script monitors the activity of these functions via the hooks. Whenever a certificate check is performed by any of the functions, the script will alter the behavior of the function by changing its return value and certain flags it uses to determine the validity of a certificate. Thus, when the function checks AntMonitor's certificate, it will always report that the certificate is valid.

\myparagraph{Decrypting Unity and Unreal.}
Since most \device{} apps are developed using either the Unity or the Unreal game engines, they use the certificate validation functions provided by these engines instead of the ones in the standard Android library.
Below, we present our implementation of certificate validation bypassing for each engine.
%For each engine, we describe how to bypass certificate validation, as described next.

For Unity, we discovered that the main function that is responsible for checking the validity of certificates is \code{mbedtls\_x509\_crt\_verify\_with\_profile()} in the Mbed TLS library, by inspecting its source code~\cite{mbedtls-cert-pinning}.
%as we observed from its source code~\cite{mbedtls-cert-pinning}.
This library is used by the Unity framework as part of its SDK. Although Unity apps and its SDK are written in C\#, the final Unity library is a C++ binary.
%Unfortunately, while the library code is open source, the entire SDK is packaged as a stripped binary file in a released app. 
%The Unity framework comes with the pre-compiled binary file of the Unity SDK.
When a Unity app is packaged for release, unused APIs and debugging symbols get removed from the Unity library's binary. %\footnote{Stripping binaries reduces app sizes by removing debugging symbols, which also makes it harder to do binary analysis. \athina{Move or remove?}}
%When packaging a released app, the framework first strips off libraries and functions irrelevant to the app from the pre-compiled binary.
%Then, the framework also removes the symbol table that contains function names and their addresses from the binary, whereas Frida scripts typically use this symbol table to locate a function in a binary file and hook into it.
This process makes it difficult to hook into Unity's functions since we cannot locate the address of a function of interest without having the symbol table to look up its address. Furthermore, since the binary also gets stripped of unused functions, we cannot rely on the debug versions of the binary to look up addresses because each app will have a different number of APIs included.
%When examining the Unity framework, we discovered that every release of the framework actually comes with the non-stripped version of the pre-compiled Unity SDK binary that still has its symbol table. 
To address this challenge, \tool{} automatically analyzes the debug versions of the non-stripped Unity binaries (provided by the Unity engine), extracts the function signature (\ie a set of hexadecimal numbers) of \code{mbedtls\_x509\_crt\_verify\_with\_profile()}, and then looks for this signature in the stripped version of the binary to find its address. 
This address can then be used to create the necessary Frida hook for an app.
The details of this automated binary analysis can be found in \appdx{\appref{}~\ref{app:binary-analysis}}.

\mycomment{
For Unreal\footnote{Unreal apps oftentimes have OBB files (\ie graphics, media files, and large program assets) that need to be pushed back upon repackaging.},}
For Unreal, we discovered that the main function that is responsible for checking the validity of certificates is the function \code{x509\_verify\_cert()} in the OpenSSL library, which is integrated as part of the Unreal SDK.
%When the Unreal engine packages a released app, it compiles this function together with the other libraries in the Unreal SDK into a binary file.
%Since OpenSSL is an open source library, 
Fortunately, the Unreal SDK binary file comes with a partial symbol table that contains the location of \code{x509\_verify\_cert()}, and thus, \tool{} can set a Frida hook for it.

%For both scenarios, when being injected to \device{} the script monitors for any API calls that trigger any of the certificate validation functions. When AntMonitor attempts to decrypt a packet using its certificate, the corresponding certificate validation function will be triggered. Simultaneously, the corresponding Frida hook will force the function to report that AntMonitor's certificate is a valid certificate and clear the flags that may indicate an invalid certificate error.

%{\ashuba[TODO: Add disclaimer here about inability to decrypt certain traffic. Perhaps add a few stats.]}

%\subsection{Dataset Summaries}
%\label{sec:dataset-summary}

\begin{comment}
    \begin{figure*}[t!]
    	\centering
        \subfigure[Top-10 eSLDs]{
    		 \includegraphics[width=.18\textwidth]{images/plots_temp/app_and_esld_third_and_platform_party_paper.pdf}
            \label{fig:top-esld-third-and-platform-party}
    	}
        \subfigure[Top-10 ATS FQDNs]{
    		 \includegraphics[width=.18\textwidth]{images/plots_temp/app_and_fqdn_ats_third_and_platform_party_paper.pdf}
            \label{fig:top-ats-third-and-platform-party}
    	}
    
    	\caption{(a) Top-10 eSLDs for platform and third-party for the Oculus and SideQuest app stores. (b) Top-10 ATS FQDNs for platform and third-party for the Oculus and SideQuest app stores.}
    	\label{fig:top-third-platform}
    \end{figure*}
\end{comment}

\mycomment{
\begin{figure}[t!]
	\centering
	\includegraphics[width=1\columnwidth]{images/plots_temp/app_and_esld_third_and_platform_party_paper.pdf}
	\caption{Top-10 eSLDs for platform and third-party for the Oculus and SideQuest app stores.}
	\label{fig:top-esld-third-and-platform-party}
\end{figure}
\begin{figure}[t!]
	\centering
	\includegraphics[width=1\columnwidth]{images/plots_temp/app_and_fqdn_ats_third_and_platform_party_paper.pdf}
	\caption{Top-10 ATS FQDNs for platform and third-party for the Oculus and SideQuest app stores.}
	\label{fig:top-ats-third-and-platform-party}
\end{figure}
}

\mycomment{
\begin{figure*}[t!]
    \begin{minipage}[b]{0.48\linewidth}
    \centering
        \includegraphics[width=0.9\textwidth]{images/plots_temp/app_and_esld_third_and_platform_party_paper.pdf}
        \caption{Top-10 eSLDs for platform and third-party for the Oculus and SideQuest app stores.}
    	\label{fig:top-esld-third-and-platform-party}
    \end{minipage}
    \hspace{0.6cm}
    \begin{minipage}[b]{0.48\linewidth}
    \centering
        \includegraphics[width=\textwidth]{images/plots_temp/app_and_fqdn_ats_third_and_platform_party_paper.pdf}
    	\caption{Top-10 ATS FQDNs for platform and third-party for the Oculus and SideQuest app stores.}
    	\label{fig:top-ats-third-and-platform-party}
    \end{minipage}
\end{figure*}
}

%\subsection{Exercising Apps}
%\label{sec:app-corpus}


\begin{comment}
Our work focuses on the official Oculus and SideQuest app stores.
As of March 2021, the official Oculus app store has 267 apps (79 free and 183 paid), and
%All of these apps are available on the Oculus store browser both on \device{} and its companion mobile app (see \secref~\ref{sec:platform-motivation}).
the SideQuest app store has 1075 apps (859 free and 218 paid).
Using the number of ratings/reviews as our criteria for popularity, we selected 3 groups of 50 apps from the following sets: (1) top free apps from the Oculus app store, (2) top paid apps from the Oculus app store, and (3) top apps from the SideQuest app store. 

We selected an equal number of paid and free apps from the Oculus app store, as we wanted to gain insight into both types equally.\footnote{Compared to previous work that mostly study free apps from the platform's official app store~\cite{androidappstudy,taintdroid,mohajeri2019watching,varmarken2020tv}, we study free and paid apps from both the official and third-party app stores.} 
If we picked top 100 apps without such proportion, paid apps would dominate our dataset (\ie 90\% paid and 10\% free apps) because paid apps tend to receive more ratings/reviews from users. 
Thus, our findings would be biased towards paid apps. 
For our selection of SideQuest apps, we did not differentiate free and paid apps since the majority of the apps are free. 
Further, we consider SideQuest apps that are below the top 50 to be of low interest, since, even in our selected top 50 apps, we found 16 apps in trial or beta versions with less than 200 ratings/reviews, indicating a small userbase.
In total, our app corpus consists of 150 apps, all of which have received an average rating of at least 3.5 stars. 
%Our automation also handles the downloading of the apps under test, including repackaging the app's APK with Frida agent and installing the repackaged APK on \device{}.

%First, we picked the top 50 free apps and the top 50 paid apps from the official Oculus app store.
%We used the number of ratings/reviews as our criteria for popularity within each subset of apps (paid and free), and we only select apps that received at least a 3.5-star rating.
%Among all the available paid apps, we selected and purchased 50 apps that: (1) had the most numbers of ratings/reviews, and (2) received at least a 3.5-star rating.

%For instance, free apps could have a different dynamics compared to paid apps in their network traffic, \eg due to advertisements and in-app purchases in free apps.

%\myparagraph{SideQuest store.}
%Next, we picked the top 50 apps from the SideQuest app store without differentiating free and paid apps since the majority of the apps are free. 
%We selected the top 50 apps based on the numbers of ratings/reviews.
%All our selected apps received at least a 4.5-star rating\footnote{Users tend to give higher ratings for apps on the SideQuest app store.}.
\end{comment}


\begin{comment}
%\myparagraph{Procedures for Data Collection.}
%In our experiment, we first install AntMonitor on \device{} and activate AntMonitor's TLS Interception feature.
%Then, we perform network traffic collection for each app.
To exercise the apps, we manually interact with each one for 7 minutes.
Although tools exist that automate the exploration of regular (non-gaming) mobile apps (\eg \cite{li2017droidbot}), automatic interaction with games is beyond the abilities of current artificial intelligence technologies.
Further, manual testing allows us to customize app exploration %based on findings in prior work~\cite{varmarken2020tv,mohajeri2019watching,shuba2020nomoats,taintdroid}.
and split our time between exploring different menus within a game and actually playing the game.
As shown by prior work, such manual testing leads to more diverse network traffic and privacy behavior~\cite{jin2018mobipurpose,recon}.
%We experiment with each app for 7 minutes---we explore the settings and (if possible) a few features of the app under test. %Simultaneously, our automation runs Frida script that performs TLS certificate pinning bypass, while AntMonitor is collecting (and decrypting) network traffic.

\end{comment}



\mycomment{
\begin{table}[t!]
	\small
	\centering
	\begin{tabularx}{\linewidth}{X | r | r}
	    \toprule
		\textbf{Description} & \textbf{Oculus} & \textbf{SideQuest}
		\\
		\midrule
		Apps & 262 & 1075  \\
		%Free & 79 & 859  \\
		%Paid & 183 & 218  \\
	    Privacy Policies & TBD & TBD \\
	    Ratings & 298K & - \\
	    Downloads & - & 6.8M \\
	    Developers & 214 & 804 \\
	    \bottomrule
	\end{tabularx}
	\caption{App store summary.}
	\label{tab:app-store-summary}
\end{table}
}

\mycomment{
\begin{table*}[t!]
	\small
	\centering
	\begin{tabularx}{\linewidth}{r | r r | r r r | r r | r r }
	    \toprule
		\textbf{App Store} &  \textbf{ Apps} & \textbf{Privacy Policy} & 
		\textbf{Unity} & \textbf{Unreal} & \textbf{Others} & 
		\textbf{Domains} & \textbf{\esld{s}} &
		\textbf{Packets} & \textbf{Flows}
		\\
		\midrule
	
		\topoculusfree & 43 & 34 & 31 & 8 & 4 & 85 & 48 & 2,818 & 2,126 \\
		
	    \topoculuspaid & 49 & 39 & 29 & 19 & 1 & 54 & 35 & 2,278 & 1,883 \\
	    
	    \topsidequest & 48 & 29 & 36 & 4 & 8 & 57 & 40 & 2,679 & 2,260 \\
	    \midrule
	    \textbf{Total} & 140 & 102 & 96 & 31 & 13 & 158 & 92 & 7,581 & 6,269 \\
	    \bottomrule
	\end{tabularx}
	\caption{Network traffic dataset summary.}
	%\todo{To RAH: Disclaimer - Packets and Flows counts consider cases where the hostname is null}}
	\label{tab:dataset-summary}
\end{table*}
}

\mycomment{
\begin{table*}[t!]
	\small
	\centering
	\begin{tabularx}{0.9\linewidth}{r | r | r r r | r r | r r | r }
	    \toprule
		\textbf{App Store} &  \textbf{ Apps} & 
		\textbf{Unity} & \textbf{Unreal} & \textbf{Others} & 
		\textbf{Domains} & \textbf{\esld{s}} &
		\textbf{Packets} & \textbf{Flows} & \textbf{Privacy Policy}
		\\
		\midrule
	
		\topoculusfree & 43 & 31 & 8 & 4 & 85 & 48 & 2,818 & 2,126 & 34 \\
		
	    \topoculuspaid & 49 & 29 & 19 & 1 & 54 & 35 & 2,278 & 1,883 & 39 \\
	    
	    \topsidequest & 48 & 36 & 4 & 8 & 57 & 40 & 2,679 & 2,260 & 29 \\
	    \midrule
	    \textbf{Total} & 140 & 96 & 31 & 13 & 158 & 92 & 7,581 & 6,269 & 102 \\
	    \bottomrule
	\end{tabularx}
	\caption{Network traffic dataset summary.}
	%\todo{To RAH: Disclaimer - Packets and Flows counts consider cases where the hostname is null}}
	\label{tab:dataset-summary}
	\vspace{-10pt}
\end{table*}
}

\mycomment{
\begin{table*}[t!]
	\small
	\centering
	\begin{tabularx}{0.8\linewidth}{r | r | r r r | r r | r r }
	    \toprule
		\textbf{App Store} &  \textbf{ Apps} & 
		\textbf{Unity} & \textbf{Unreal} & \textbf{Others} & 
		\textbf{Domains} & \textbf{\esld{s}} &
		\textbf{Packets} & \textbf{TCP Flows}
		\\
		\midrule
	
		\topoculusfree & 43 & 31 & 8 & 4 & 85 & 48 & 2,818 & 2,126 \\
		
	    \topoculuspaid & 49 & 29 & 19 & 1 & 54 & 35 & 2,278 & 1,883 \\
	    
	    \topsidequest & 48 & 36 & 4 & 8 & 57 & 40 & 2,679 & 2,260 \\
	    \midrule
	    \rowcolor{brandeisblue!10}
	    \textbf{Total: \textit{All Stores}} & 140 & 96 & 31 & 13 & 158 & 92 & 7,775 & 6,269 \\
	    \bottomrule
	\end{tabularx}
	\caption{Network traffic dataset summary.}
	%\todo{Need to update these packets and network flows}
	%\todo{To RAH: Disclaimer - Packets and Flows counts consider cases where the hostname is null}}
	\label{tab:dataset-summary}
\end{table*}
}





\subsection{Network Traffic Dataset}
\label{sec:network-traffic-dataset}
%\myparagraph{Oculus-Free-Top50.}


\subsubsection{Raw Network Traffic Data}
\label{sec:network-traffic-dataset-raw}

\minorrevision{We used \tool{} to collect network traffic for 140\footnote{\minorrevision{The remaining 10 apps were excluded for the following reasons: (1) six apps could not be repackaged;
%due to some missing configuration files;
%Due to limitations of the tools we use (see \secref{}~\ref{sec:limitations}), we had to exclude
%(we further discuss this limitation in \secref{}~\ref{sec:limitation-conclusion}); 
(2) two apps were browser apps, which would open up the web ecosystem, diverting our focus from VR; (3) one app was no longer found on the store---we created our lists of top apps 
%in February 2021 and we could no longer find the app on the Oculus store during our experiment in March and April 2021; 
one month ahead of our experiments;
and (4) one app could not start on the \device{} even without any of our modifications.}} apps in our corpus}
during the months of March and April 2021.
To exercise these 140 apps and collect their traffic, we manually interacted with each one for seven minutes.
Although there are existing tools that automate the exploration of regular (non-gaming) mobile apps (\eg \cite{li2017droidbot}), automatic interaction with a variety of games is an open research problem. %currently beyond the abilities of artificial intelligence technologies.
Fortunately, manual testing allows us to customize app exploration %based on findings in prior work~\cite{varmarken2020tv,mohajeri2019watching,shuba2020nomoats,taintdroid}.
and split our testing time between exploring menus within the app to cover more of the potential behavior, and actually playing the game, which better captures the typical usage by a human user. As shown by prior work, such testing criteria lead to more diverse network traffic and reveal more privacy-related data flows~\cite{jin2018mobipurpose,recon, varmarken2020tv}. 
%We experiment with each app for 7 minutes---we explore the settings and (if possible) a few features of the app under test. %Simultaneously, our automation runs Frida script that performs TLS certificate pinning bypass, while AntMonitor is collecting (and decrypting) network traffic.
%\athina{[This is a first comprehenesive.... dataset??]}
Although our methodology might not be exhaustive, it is inline with prior work~\cite{mohajeri2019watching, varmarken2020tv}.

%
%Only 102 out of 140 apps have privacy policy texts.
\tabref{}~\ref{tab:dataset-summary} presents the summary of our network traffic dataset.
We discovered 158 domains and 92 \esld{}s in \tcpflowtotal{} TCP flows that contain \packettotal{} packets.
Among the 140 apps, 96 were developed using the Unity framework, 31 were developed using the Unreal framework, and 13 were developed using other frameworks.
\vspace{-5pt}

%For the top 50 free apps on the official Oculus app store, we successfully collected network traffic for 43 out of 50 apps. We excluded the other 7 apps: (1) 3 apps are Oculus system apps (\eg web browsers), (2) 3 apps could not be repackaged with Frida agent (\eg a Kotlin app), and (3) 
%We found that only 34 out of 43 apps have privacy policy texts. Out of 43 apps, 31 are Unity apps, 8 are Unreal apps, and 4 apps were developed using other frameworks (\eg Xamarin framework).
%In the collected traffic of the 43 apps, we discovered 85 domains with 48 eSLDs. In total, there are 2,818 packets in 2,126 flows.

%\myparagraph{Oculus-Paid-Top50.}
%For the top 50 paid apps on the official Oculus app store, we successfully collected network traffic for 49 apps.
%We excluded 1 app that we could not repackage with Frida agent.
%Surprisingly, we found that only 39 out of 49 apps have privacy policies. Even though the Oculus store seems to require an official app to have its privacy policy linked in the app's game profile, many of the apps do not have the link posted on their profile or they post a broken link. We also tried to visit the official websites, but we still did not find the privacy policies for these official apps.
%Out of 49 apps, 29 are Unity apps, 19 are Unreal apps, and 1 was developed using other frameworks.
%In the collected traffic of the 49 apps, we found 54 domains with 35 eSLDs. Overall, there are 2,278 packets in 1,883 flows.

%\myparagraph{SideQuest-Top50.}
%For the top 50 apps on the SideQuest app store, we successfully collected network traffic for 48 apps.
%We excluded 2 apps because 1 app could not be repackaged with Frida agent and the other 1 app did not even run on Quest 2---it might not be maintained anymore by the developer.
%Although a lot of apps in this store do not have privacy policies since the majority are in demo version, we found that 29 out of 48 apps actually have privacy policies.
%Out of 48 apps, 36 are Unity apps, 4 are Unreal apps, and 8 were developed using other frameworks---a lot of these are old computer games that are ported to run on Oculus headsets.
%In the collected traffic of the 48 apps, we found 57 domains with 92 eSLDs. Overall, there are 2,679 packets in 2,260 flows.



\begin{table}[t!]
	\tabletextsize
	\begin{tabularx}{\columnwidth}{r | r | r r | r r }
	    \toprule
		\textbf{App Store} &  \textbf{ Apps} & 
		\textbf{Domains} & \textbf{\esld{s}} &
		\textbf{Packets} & \textbf{TCP Fl.}
		\\
		\midrule
	
		\topoculusfree & 43 & 85 & 48 & 2,818 & 2,126 \\
		
	    \topoculuspaid & 49 & 54 & 35 & 2,278 & 1,883 \\
	    
	    \topsidequest & 48 & 57 & 40 & 2,679 & 2,260 \\
	    \midrule
	    \rowcolor{brandeisblue!10}
	    \textbf{Total} & 140 & 158 & 92 & \packettotal{} & \tcpflowtotal{} \\
	    \bottomrule
	\end{tabularx}
	\vspace{-5pt}
	\caption{\textbf{Network traffic dataset summary.} Note that the same domains and eSLDs can appear across the three groups of ``App Store'', so their totals are based on unique counts.}
	%\todo{Need to update these packets and network flows}
	%\todo{To RAH: Disclaimer - Packets and Flows counts consider cases where the hostname is null}}
	\label{tab:dataset-summary}
	\vspace{-10pt}
\end{table}


\begin{figure*}[t!]
    \centering
    %\captionsetup[subfigure]{labelformat=empty}
    %\vspace{-10pt}
    \begin{subfigure}{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/plots_temp/app_and_esld_third_and_platform_party_paper.pdf}
        \vspace{-2em}
        \caption{}
        \label{fig:top-esld-third-and-platform-party}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/plots_temp/app_and_fqdn_ats_third_and_platform_party_paper.pdf}
        \vspace{-2em}
        \caption{}
        \label{fig:top-ats-third-and-platform-party}
    \end{subfigure}
    \vspace{-5pt}
    \caption{\textbf{Top-10 platform and third-party (a) eSLDs  and (b) ATS FQDNs.} They are ordered by the number of apps that contact them. Each app may have a few first-party domains: we found that 46 out of 140 (33\%) apps contact their own eSLDs.}
    \label{fig:top-esld-ats}
    \vspace{-10pt}
\end{figure*}

%\subsection{\tool{} Dataset}
\subsubsection{Network Data Flows Extracted}
\label{sec:labeling-data-flow}
%Our \dataset{} is derived from the 
We processed the raw \netdataset{} and identified \dataflowtotal{} data flows: \dataflow{}. %\footnote{Purpose for each data flow is extracted from privacy policy (see \secref{}~\ref{sec:polisis-context}).} 
Next, we describe our methodology for extracting that information.

\myparagraph{App names.}
For each network packet, the app name is obtained by AntMonitor~\cite{shuba2016antmonitor}. This feature required a modification to work on Android 10, as described in
\appdx{\appref{}~\ref{app:antmonitor-improvement}}.

% using android APIs: looking up the UID, and eventually the package name, of the app responsible for the connection the packet belongs to.

%the network packets’ source and destination IPs and port numbers in the list of active connections in /proc/net, which provides the UIDs of apps responsible for each connection. Given a UID, we get the corresponding package name using Android APIs.”

\myparagraph{Data types.}
%The data types found in the data flows extracted from our network traffic dataset
The data types we extracted from our network traffic dataset are listed in \tabref{}~\ref{tab:pii-summary} and can be categorized into roughly three groups. 
First, we find personally identifiable information (\textit{PII}), including: user identifiers (\eg Name, Email, and User ID), device identifiers (Android ID, Device ID, and Serial Number), Geolocation, \etc 
Second, we found system parameters and settings, whose combinations are known to be used by trackers to create unique profiles of users~\cite{mohajeri2019watching, moz-fingerprinting}, \ie \textit{Fingerprints}. 
Examples include various version information (\eg{} Build and SDK Versions), Flags (\eg{} indicating whether the device is rooted or not), Hardware Info (\eg{} Device Model, CPU Vendor, \etc), Usage Time, \etc
Finally, we also find data types that are unique to VR devices (\eg{} VR Movement and VR Field of View) and group them as \textit{VR Sensory Data}. 
These can be used to uniquely identify a user or convey sensitive information---the VR Play Area, for instance, can represent the actual area of the user's household.
%Further, we consider VR Play Area as possible PII, as it represents the actual play area of a user's household. 
%We deem the others as information that can be joined for fingerprinting.




We use several approaches to find these data types in  HTTP headers and bodies, and also in any raw TCP segments that contain ASCII characters.
First, we use string matching to search for data that is static by nature. 
For example, we search for user profile data (\eg{} User Name, Email, \etc) using our test \oculusvr{} account and for any device identifiers (\eg{} Serial Number, Device ID, \etc) that can be retrieved by browsing the \device{} settings.
%The common approach is to find keywords or exact values to match within our \netdataset{}~\cite{shuba2018nomoads, recon}; specifically, URL components (\eg{} paths and query parameters), HTTP headers, and HTTP request body. 
%
In addition, we search for their MD5 and SHA1 hashes.
Second, we utilize regular expressions to capture more dynamic data types. For example, we can capture different Unity SDK versions using \verb!UnityPlayer/[\d.]+\d!.
Finally, for cases where a packet contains structured data (\eg URL query parameters, HTTP Headers, JSON in HTTP body, \etc), we split the packet into key-value pairs and create a list of unique keys that appear in our entire network traffic dataset.
We then examine this list to discover keys that can be used to further enhance our search for data types.
For instance, we identified that the keys ``user\_id'' and ``x--playeruid'' can be used to find User IDs. 
\appdx{\appref{}~\ref{app:extracting-data-types-appendix}} provides more details on our data types. % and how we extract them.
%
%Data types can be a combination of other data types. Hardware Info comprises of Device Model, CPU, GPU, and Screen Resolution information. 





%\vspace{-40pt}

\myparagraph{Destinations.}
To extract the destination fully qualified domain name (FQDN), we use the HTTP Host field and the TLS SNI (for cases where we could not decrypt the traffic). 
Using tldextract, %~\cite{tldextract} 
we also identify the effective second-level domain (eSLD) and use it to determine the high level organization that owns it via Crunchbase. %~\cite{crunchbase-homepage, varmarken2020tv}.
We also adopt similar labeling methodologies from~\cite{varmarken2020tv} and~\cite{andow2020actions} to categorize each destination as either \emph{first-}, \emph{platform-}, or \emph{third-}party.
To perform the categorization, we also make use of collected privacy policies (see \figref{}~\ref{fig:our-work} and \secref{}~\ref{sec:privacy-policy}), as described next.
First, we tokenize the domain and the app's package name.
We label a domain as first-party if the domain's tokens either appear in the app's privacy policy URL or match the package name's tokens.
If the domain is part of cloud-based services (\eg \textit{vrapp.amazonaws.com}), we only consider the tokens in the subdomain (\textit{vrapp}). 
Second, we categorize the destination as platform-party if the domain contains the keywords ``oculus'' or ``facebook''.
Finally, we default to the third-party label.
This means that the data collection is performed by an entity that is not associated with app developers nor the platform, and the developer may not have control of the data being collected.
The next section presents further analysis of the destination domains.


%begin{enumerate}
\mycomment{
\squishcount
    \item \textit{FQDNs and eSLDs}: From the domain that we collect, we use tldextract~\cite{tldextract} to determine the FQDN and eSLD forms that receive the data type. We use Crunchbase~\cite{crunchbase-homepage} to identify the high level organization that owns them. 
    \item \textit{Entities}: Entities are names of companies and other organizations. We need to translate domains to entities in order to associate data flows with disclosures in the privacy policies in Section~\ref{sec:privacy-policy}.

    Same as~\cite{andow2020actions}, we use a manually-crafted list of domain-to-entity mapping to determine which entity that each domain belongs to. For example, \texttt{*.playfabapi.com} is a domain of the entity Playfab. We started from PoliCheck's mapping, and added missing domains and entities to it. We visited each new domain and read the information on the website to determine its entity. If we could not determine the entity for a domain, we labeled its entity as \textit{unknown third party}.

    \item \textit{Party Categorization}: To provide context for how apps can expose data to external destinations, we combine the labeling methodology from ~\cite{varmarken2020tv} and~\cite{andow2020actions}, which categorize each packet as either \emph{first}, \emph{third}, or \emph{platform-party}. We apply this consistently through Sections~\ref{sec:ats-pii-analyses} and~\ref{sec:privacy-policy}.

    First-party label means that the app's data collection is performed by its developer. First, we compare the domain to the app's privacy policy URL. If the domain is part of cloud-based services (\eg \textit{amazonaws.com}), we then rely on its subdomain; otherwise, we rely on its eSLD. If the string appears in the privacy policy URL or in the app's package name, we will label it as a first-party. Second, we compare the outgoing domain with the app's package name. We tokenize the package name and see if the tokens appear in the eSLD of the domain.
    
    Platform-party label is applied when an app relies on a system app to contact a platform-party domain. Recall that~\cite{shuba2016antmonitor} can identify when a system app is making the outgoing request. We categorize a packet as platform-party if the system app makes a request to a domain that has keywords \textit{facebook}, \textit{oculus}, \textit{android}, and \textit{qualcomm}. We identify these keywords by inspecting the list of system apps for the Oculus.
    
    Otherwise, we default to third-party label. This means that the data collection is performed by an entity that is not associated with app developers nor the platform. In such cases, the developer may not have total control of the data being collected.
    %Even if the developer chooses to use the service, we still treat it as third-party---the developer do 
%\end{enumerate}
\countend
}


\mycomment{
In summary, for each packet:
\begin{itemize}
    \item \textit{First-party.} This means that the data goes to the app developers. First, we compare the domain to the app's privacy policy URL. If the domain is part of cloud-based services like \textit{amazonaws.com}, then we rely on its subdomain; otherwise, we rely use its eSLD. We see if the string appears in the privacy policy URL. If yes, we label it as a first-party. Otherwise, we see if the string appears in the app's package name. If yes, we label it as a first-party. Second, we compare the outgoing domain with the app's package name. We tokenize the package name and see if the tokens appear in the eSLD of the domain.
    \item \textit{Platform-party.} This represents when an app relies on a system app to contact a platform-party domain. Recall that~\cite{shuba2016antmonitor} can identify when a system app is making the outgoing request. We categorize a packet as platform-party if the system app makes a request to a domain that has keywords \textit{facebook}, \textit{oculus}, \textit{android}, and \textit{qualcomm}. We identify these keywords by inspecting the list of system apps for the Oculus.
    \item \textit{Third-party.} Otherwise, we default to third-party. This means that the data is being sent to an entity that is not associated with app developers. Even if the developer chooses to use the service, we still treat it as third-party, since the app developers do not have total control of the data being collected.

\end{itemize}
}

%\subsection{Summary} \label{data-collection-summary}
%\todo{To RAH: add some summary/transition to next main section?}



==> VR Project (USENIX Security 2022)/discussion.tex <==
\minorrevision{
\section{Discussion}
\label{sec:discussion}
}

%In this section, we discuss further noteworthy findings from our study.  We highlight the uniqueness of VR in \secref{}~\ref{sec:major-findings} and
%discuss threats to the validity of our study in \secref{}~\ref{sec:threats-to-validity}, 
%make recommendations based on our study in \secref{}~\ref{sec:recommendations}.
%, and outline responses we received from developers after we notified them about our findings in \secref{}~\ref{sec:responses}.

%We reflect on noteworthy findings obtained from our paper and discuss their implications for Oculus and VR in general.

\minorrevision{
\subsection{VR-Specific Considerations}
\label{sec:major-findings}
VR tracking has unique aspects and trends compared to other ecosystems, including but not limited to the following.
}

\minorrevision{
%\myparagraph{Immersive Ads.} 
\myparagraph{VR ads.} The VR advertising ecosystem is currently at its infancy. Our analysis of destinations from the network traffic revealed that ad-related activity was missing entirely from \oculusvr{} at the time of our experiments. Facebook recently started testing on-device ads for Oculus in June 2021 ~\cite{oculus-ads}.
Ads on VR platforms will be immersive experiences instead of flat visual images; for example, Unity uses separate virtual rooms for ads~\cite{unity-virtual-room-ads}. We expect that tracking will further expand once advertising comes into VR (\eg to include tracking how users interact and behave within the virtual ad space). 
As VR advertising and tracking evolve, our \tool{} methodology, system, and datasets will continue to enable analysis that was not previously possible on any VR platforms.}


\minorrevision{
\myparagraph{Comparison to other ecosystems.} Our analysis showed that the major players in the
\oculusvr{} tracking ecosystem are currently Facebook and Unity (see \figref{}~\ref{fig:top-esld-ats} and~\ref{fig:flow-to-policy-consistency-analysis}). The more established ecosystems such as mobile and Smart TVs are dominated by Alphabet ~\cite{kollnig2021ios, varmarken2020tv}; they also have a more diverse playing field of trackers (\eg{} Amazon, Comscore Inc., and Adobe)---spanning hundreds of tracking destinations~\cite{kollnig2021ios, varmarken2020tv, shuba2020nomoats}. \oculusvr{} currently has only a few players (\eg Facebook, Unity, Epic, and Alphabet). \tool{} can be a useful tool for continuing the study on this developing ecosystem. %develop and potentially expand to more organizations starting to track \oculusvr{} users in the future. 
}




%\todo{Potentially add more references above to other ecosystems (Alexa, IoT)?} \todo{And add reference to other mobile SmartTV papers if appropraite. Note that the Han2013 reference includes iOS, so please do not remove}


\minorrevision{
\myparagraph{Sensitive data.} 
Compared to other devices, such as mobile, Smart TVs and IoT, the type of data that can be collected from a VR headset is arguably more sensitive. For example, \oculusvr{} has access to various biometric information (\eg pupillary distance, hand geometry, and body motion tracking data) that can be used to identify users and even infer their health~\cite{oculus-move}. A study by Miller \etal~\cite{oculus-privacy-3} revealed the feasibility of identifying users with a simple machine learning model using less than five minutes of body motion tracking data from a VR device. Our experiments found evidence of apps collecting data types that are unique to VR, including biometric-related data types (see \secref{}~\ref{sec:labeling-data-flow}). While the numbers we found are small so far, with the developing VR tracking ecosystem, it is important to have a system such as \tool{} to detect the increasing collection of sensitive data over time.
}

\begin{comment}
\rahmadi{
Third, our findings also include data types that are unique to VR devices (see \secref{}~\ref{sec:labeling-data-flow}). In addition to the VR Play Area that can represent the actual area of the user's household, other sensory data can present more privacy threat to users: a study from Miller \etal aptly illustrates such threat~\cite{oculus-privacy-3}. The authors conducted a study that involved 511 participants and found that a simple machine learning model can be used to identify participants using less than 5 minutes of body motion tracking data (from a VR device) with more than 95\% accuracy.
During the time that we conducted our network traffic collection, we already found that biometric information (\eg pupillary distance) was collected by some VR apps. Thus, we postulate a trend that more biometric information will be collected in the future---it is possible that future VR devices incorporate more types of sensors.
}
\end{comment}
%%

%\todo{Suggestions from ashuba: Add notes about unique info available on VR. Some we found being sent now, others may be potentially collected in the future. Such info is not available on TVs and mobile devices. Cite and discuss https://www.nature.com/articles/s41598-020-74486-y}


\minorrevision{
\myparagraph{Generalization.}
%\paragraph{Internal Validity.}
Within \oculusvr{}, we only used \tool{} to analyze 140 apps in our corpus. However, we believe that it can be applied  to other \oculusvr{} apps, as long as they are created according to \oculusvr{} standards.
%\footnote{\athina{We found six apps whose APKs were missing certain components in their APKs when being repackaged and, thus, we had to exclude them (see \secref{}~\ref{sec:network-traffic-dataset-raw}).}
%\myparagraph{External Validity.}
%Although we developed and tested \tool{} on the \oculusvr{} platform, 
Beyond \oculusvr{}, the network traffic analysis and network-to-policy consistency analysis can also be applied to other platforms, as long as their network traffic can be decrypted, as was the case with prior work on Android, Smart TV, \etc~\cite{shuba2016antmonitor,razaghpanah2018apps,mohajeri2019watching,varmarken2020tv}.}



\minorrevision{
\subsection{Recommendations}
\label{sec:recommendations}
Based on our findings, we provide recommendations for the \oculusvr{} platform and developers to improve their data transparency practices.}

\minorrevision{
\myparagraph{Provide a privacy policy.}
We found that 38 out of the 140  popular apps, out of which 19 are from the Oculus app store,  did not provide any privacy policy at all.
%
Furthermore, 97\% of inconsistent data flow disclosures were due to omitted disclosures by these 38 apps missing privacy policies (see \secref{}~\ref{sec:privacy-policy}).
We recommend that the \oculusvr{} platform require developers to provide a privacy policy for their apps, especially those available on the official Oculus app store.
}

\minorrevision{
\myparagraph{Reference other parties' privacy policies.} 
Developers are not the only ones collecting data during the usage of an app: third-parties (\eg{} Unity, Microsoft) and platform-party (\eg{} Oculus/Facebook) can also collect data.  We found that 81 out of 102 app privacy policies did not reference policies of third-party  libraries used by the app. We recommend that developers reference third-party and platform-party privacy policies. If they do that, then the consistency of disclosures will be quite high: up to 74\% of data flows in the network traffic we collected (see~\secref{}~\ref{sec:policheck-results}). This indicates that, at least at this early stage, the VR ecosystem is better behaved than the mobile tracking ecosystem. 
}

\minorrevision{
\myparagraph{Notice and consent.}
We found that fewer than 10 out of 102 apps that provide a privacy policy explicitly ask users to read it and give consent to data collection (\eg{} for analytics purposes) upon first opening the app.
We recommend that developers provide notice and ask for users' consent (\eg when a user launches the app for the first time) for data collection and sharing, as required by privacy laws such as GDPR~\cite{gdpr-implementation}.}
%\todo{We should include related work here about why consent is important (can we say that Android already does this?)}

%For better data transparency, developers should reference third-parties (that are utilized within the app) and  platform-party privacy policies as well. 

\begin{comment}
\rahmadi{
\myparagraph{Opening Oculus OS for Research}
We recommend that \oculusvr{} open the Oculus OS to foster a trustworthy platform. Unlike \rahmadi{Android} platforms that can be rooted, \oculusvr{} has resisted against efforts to root the Oculus OS~\cite{failedjailbreak}, while also requiring users to login with their Facebook account.} This prevents external parties, \rahmadi{such as} researchers, from auditing the device \rahmadi{(\eg network-to-policy consistency analysis)} and raises concerns from consumers about using \oculusvr{} devices~\cite{adams2018ethics}. This practice is contradictory to \oculusvr{}'s advocacy for side-loading of unofficial apps, which may need additional vetting of data collection practices.
\end{comment}

%\todo{Add user recommendation?}

\minorrevision{
\myparagraph{Notifying developers.} We contacted Oculus as well as the developers of the 140 apps that we tested. We provided courtesy notifications of the specific data flows and consistency we identified in their apps, along with recommendations. We received 24 responses (see the details \appdx{in~\appref{}~\ref{sec:responses}}).}
\minorrevision{Developers were, in general, appreciative of the information and willing to adopt recommendations to improve their privacy policies. Several indicated they did not have the training or tools to ensure consistent disclosures.}




\begin{comment}
\myparagraph{Limitations.}
%\textit{Network Traffic Methodology.} 
We manually test every app, which is an open challenge especially for VR apps where the camera must be moved to see an object before interacting with it. Next, we only test each app for seven minutes.
Thus, the network traffic we collected is not exhaustive. However, we note that this is inline with prior work~\cite{mohajeri2019watching, varmarken2020tv}. Following guidelines from~\cite{varmarken2020tv}, we explore menus and play the game during each experiment to trigger as much network traffic as possible.
%
We cannot decrypt much of the platform traffic since Oculus is a closed platform. 
%The platform uses a function in the Oculus SDK to perform certificate validation --- we do not have access to the source code (as we do for \code{Mbed TLS} and \code{OpenSSL}) and the Oculus SDK is also compiled into stripped binary files.
%Overall, we decrypted over 50\% of the app traffic---we discovered that much of the app traffic also uses the Oculus SDK, whose source code we do not have access to.

%Some apps in our corpus are problematic. For instance, 6 apps could not be repackaged properly. We discovered that, for example, the app's APK was missing a configuration file is usually manipulated to force the app to load Frida library at runtime.
%We also found apps that are not fully functional (\eg fail to login) due to our use of Frida and AntMonitor to collect network traffic.
%Nevertheless, we still count these apps as functional if AntMonitor still collects network traffic.
%\textit{Policy Analysis.} 
We also discovered limitations in \policheck{}. Although we could already improve certain aspects of \policheck{}, we could not fix its limitations in the NLP model or the algorithm in the source code without altering the core functionality of \policheck{}.

\myparagraph{Future Directions.}
%We believe that our methodology and collection of tools that we have integrated in \tool{} can be applied for other platforms and domains.
%The framework ``Privacy in Context'' (in the form of the tuple \dataflowtuple{}) that we have defined and applied in the VR domain is a more comprehensive means of viewing data privacy than just observing the network traffic or privacy policy separately. {\todo{\hieu{companion app, other third party app stores like SteamVR, Built-in Apps (Oculus Move)}}}
Future work on \oculusvr{} include further study and evaluation on \oculusvr{} companion mobile app, built-in apps (\eg Oculus Move), and other third-party app stores.
As suggested by our findings, future research in privacy policies should look into multiple privacy policies that are relevant when performing app study in other platforms.
Although \tool{} is created for \oculusvr{}, we believe that our methodology can be replicated for other domains and platforms in future work.

%\todo{This is not clear. Just say it outright how it helps generalize to other domains.}
\end{comment}

\mycomment{
\myparagraph{Limitations.}
%\textit{Network Traffic Methodology.} 
We manually test every app, which is an open challenge especially for VR apps where the camera must be moved to see an object before interacting with it. Next, we only test each app for seven minutes.
Thus, the network traffic we collected is not exhaustive. However, we note that this is inline with prior work~\cite{mohajeri2019watching, varmarken2020tv}. Following guidelines from~\cite{varmarken2020tv}, we explore menus and play the game during each experiment to trigger as much network traffic as possible.
%
We cannot decrypt much of the platform traffic since Oculus is a closed platform. 
%The platform uses a function in the Oculus SDK to perform certificate validation --- we do not have access to the source code (as we do for \code{Mbed TLS} and \code{OpenSSL}) and the Oculus SDK is also compiled into stripped binary files.
%Overall, we decrypted over 50\% of the app traffic---we discovered that much of the app traffic also uses the Oculus SDK, whose source code we do not have access to.

%Some apps in our corpus are problematic. For instance, 6 apps could not be repackaged properly. We discovered that, for example, the app's APK was missing a configuration file is usually manipulated to force the app to load Frida library at runtime.
%We also found apps that are not fully functional (\eg fail to login) due to our use of Frida and AntMonitor to collect network traffic.
%Nevertheless, we still count these apps as functional if AntMonitor still collects network traffic.
%\textit{Policy Analysis.} 
We also discovered limitations in \policheck{}. Although we could already improve certain aspects of \policheck{}, we could not fix its limitations in the NLP model or the algorithm in the source code without altering the core functionality of \policheck{}.
}

\mycomment{
\begin{itemize}
    \item Our testing methodology is limited in that (1) it is not automated because of the nature of a VR headset that requires a real user; (2) a human tester will not be able to cover all the features in an app, especially since we also limit the test time to 7 minutes per app---these apps are complex games that actually require hours of gameplay (unlike traditional Android apps which have fairly limited numbers of features, where users can interact directly with the apps through menu options and buttons).
    \item When the app developer does not explicitly state their privacy policy, we may have missed it when we do not find it easily. Some developers are vague about their privacy policy. Sometimes, some developers also revert it to the privacy policy from third-party libraries or Facebook/Oculus.
    \item We cannot look into the stack trace since the Unity and Unreal apps use stripped binaries that do not have symbols (unlike traditional Android apps that run on a JVM whose stack trace can be easily obtained through Frida).
    \item We can decrypt system apps with only certain API levels. We can decrypt certain Unity and Unreal traffic by bypassing: (1) SSL pinning in the \code{mbedtls} library, (2) SSL pinning in the OpenSSL library---both libraries are embedded in the binaries for Unity and Unreal apps. Unfortunately, certain traffic, such as the one that contains communication between the device and Facebook cannot be decrypted---we suspected that this originates from the \code{libovrplatform.so} binary which contains the Oculus Platform SDK from Facebook.
    \item Broken apps after we use our traffic collection technique: 1) RecRoom issue: can't login; 2) VrChat/Youtube: can't go beyond the title screen. 3) Browser apps like FireFox cannot start at all.
    \item We only focus on social apps and games (Unity and Unreal), so we skip apps such as browsers.
    \item PoliCheck's NLP model is limited in recognizing the intent of data collection and sharing in privacy policy texts. It cannot parse more complex sentences correctly, especially if the intent is expressed in multiple sentences. It typically is successful when the sentence is in the format of \emph{we collect/share your A, B, C, etc.} with \emph{A, B, C, etc.} being data types.
\end{itemize}
}

\mycomment{
\myparagraph{Future Directions.}
We believe that our methodology and collection of tools that we have integrated in \tool{} can be applied for other platforms and domains.
The framework ``Privacy in Context'' (in the form of the tuple \dataflowtuple{}) that we have defined and applied in the VR domain is a more comprehensive means of viewing data privacy than just observing the network traffic or privacy policy separately. {\todo{\hieu{companion app, other third party app stores like SteamVR, Built-in Apps (Oculus Move)}}}
\athina{
Although \tool{} is created for \oculusvr{}, we believe that our methodology can be replicated for other domains and platforms in future work. }
%\todo{This is not clear. Just say it outright how it helps generalize to other domains.}

\myparagraph{Recommendations.} 
{\todo{\hieu{Facebook opening up Oculus for researchers to audit platform network traffic, developers add third- and platform-party privacy links. Platform and Third party privacies should be more exact on their data collection (aka less vagueness).}}}
}

==> VR Project (USENIX Security 2022)/introduction.tex <==

\mycomment{
\begin{figure*}[ht!]
	\centering
	\includegraphics[width=0.8\textwidth]{images/plots_temp/Paper_Workflow_contributions.pdf}
	\caption{\tool{} Workflow: TBD}
	\label{fig:main-workflow}
\end{figure*}
}

\section{Introduction}
\label{introduction}
Virtual reality (VR) technology has created an emerging market: VR hardware and software revenues are projected to increase from \$800 million in 2018 to \$5.5 billion in 2023~\cite{vr-market}. 
%
%VR is considered the new platform for app developers~\cite{new-vr-platform}. 
%
Among VR platforms, Oculus VR (\oculusvr{}) is a pioneering, and arguably the most popular one: within six months since October 2020, an estimated five million \device{} headsets were sold~\cite{oculus-acquisition, oculus2-popular}.
\mycomment{
Oculus VR (\oculusvr{}), in particular, is a pioneering, and arguably the most popular, VR platform: within six months since October 2020, an estimated five million \device{} headsets were sold~\cite{oculus-acquisition,fb-q1-2021-earnings, oculus2-popular, oculus2-sales}.}
%
VR technology enables a number of applications, including recreational games, physical training, health therapy, and many others~\cite{vr-use-cases}. 


VR also introduces privacy risks: some are similar to those on other Internet-based platforms (\eg mobile phones~\cite{androidappstudy,taintdroid}, IoT devices~\cite{iotsok,iotsecurity}, and Smart TVs~\cite{mohajeri2019watching,varmarken2020tv}), but others are unique to VR. %  
%In addition, VR has its own unique characteristics: oalso has access to sensitive user data and it has its own unique characteristics as a platform.
%
For example, VR headsets and hand controllers %to interact with the virtual environment visible through the headset.
%The headset and controllers 
are equipped with sensors that may collect data about the user's physical movement, body characteristics and activity, voice activity, hand tracking, eye tracking, facial expressions, and play area~\cite{oculus-privacy-1,oculus-privacy-3}, which may in turn reveal information about our physique, emotions, and home.
\mycomment{For example, VR headsets and hand controllers %to interact with the virtual environment visible through the headset.
%The headset and controllers 
 are equipped with sensors that may collect data about the user's physical movement, body characteristics and activity, voice activity, hand tracking, eye tracking, facial expressions, and play area~\cite{oculus-privacy-1,oculus-privacy-2,oculus-privacy-3}, which may in turn reveal information about our physique, emotions, and home.}
%Since this usage model does not exist on other platforms, the privacy aspects of the collection of these new data types have not been widely studied by the research community.
The privacy aspects of VR platforms are currently not well understood~\cite{adams2018ethics}.
%Our work presents the first comprehensive study and analyses on the privacy aspects of the VR platform.

%To the best of our knowledge, this paper is the first wide-scale, comprehensive measurement and characterization of various privacy aspects of VR apps and platform from a combined technical and privacy policy point of view. 
%These include: the Advertising and Tracking \athina{(a.k.a. ATS)} ecosystem in VR, personally identifiable information (PII) exposures, privacy policies and their consistency with the systems' behavior. 
%We leverage the most popular platform, \oculusvr{}, and use its latest device, \device{},
%---recently dubbed ``the best standalone VR headset'' in 2021~\cite{oculus2-popular, oculus2-sales}---
%
%to experiment with 150 most popular apps---paid and free---on both the official Oculus app store and SideQuest (a third-party app store endorsed by Oculus~\cite{oculus-sidequest}). %We use its latest device, 
%Compared to previous work that mostly study free apps from the platform's official app store~\cite{androidappstudy,taintdroid,mohajeri2019watching,varmarken2020tv}, we study free and paid apps from both the official and third-party app stores.
%We present a comprehensive analysis and evaluation of various privacy aspects of VR apps, including the ATS ecosystem, PII exposures, and privacy policies on the Oculus platform. 
%We study three privacy aspects of the \oculusvr{} platform: (1) advertising and tracking services (\ie ATSes); (2) the exposures of ``data types'': personally identifiable information (PII), information that can be combined for fingerprinting, and VR sensor data; and (3) privacy policy consistency and data collection purposes.
\begin{figure*}[t!]
	\centering
	\vspace{-5pt}
	\includegraphics[width=0.9\linewidth]{images/paper_workflow.pdf}
	\vspace{-5pt}
	\caption{\textbf{Overview of \tool{}.}	We select the most popular apps from the official Oculus and SideQuest app stores. 
    First,	we experiment with them and analyze their {\bf network traffic:} (1) we obtain raw data in PCAPNG and JSON; (2) we extract data flows \dataflowtuple{}; and (3) we analyze them \wrt{} data types and ATS ecosystem. 
	Second, we analyze the same apps' (and their used libraries') {\bf privacy policies}: (4) we build VR-specific data and entity ontologies, informed both by network traffic and privacy policy text; and (5) we extract collection statements \polichecktuple{}  from the privacy policy. Third, we {\bf compare the two}: (6) using our improved \policheck{}, we map each data flow to a collection statement, and we perform network-to-policy consistency analysis. Finally,  (7) we  translate the sentence containing the collection statement into a text segment that \polisys{} can use to extract the data collection purpose. The end result is that data flows, extracted from network traffic, are augmented with additional {\bf context}, such as consistency with policy and purpose of collection. %, extracted from privacy policy and ATS analyses. 
	%Finally, data flow is represented as \dataflowtuple{}. 
	}
	\label{fig:our-work}
	\vspace{-10pt}
\end{figure*}

 


To the best of our knowledge, our work is the first large scale, comprehensive measurement and characterization of privacy aspects of \oculusvr{} apps and platform, from a combined network and privacy policy point of view. We set out to characterize how sensitive information is collected and shared in the VR ecosystem, in theory (as described in the privacy policies) and in practice (as exhibited in the network traffic generated by VR apps). We center our analysis around the concept of {\em data flow}, which we define as the tuple \dataflowtuple~extracted from the network traffic. First, we are interested in the sender of information, namely the VR \emph{app}.  
Second, we are interested in the exposed {\em data types}, including personally identifiable information (PII), device information that can be used for fingerprinting, and VR sensor data. 
Third, we are interested in the recipient of the information, namely the {\em destination} domain, which we further categorize into entity or organization, first \vs{} third party \wrt{} the sending app, and ads and tracking services (ATS).  
%Finally, we identify the {\em purpose} of data flow, which affects whether it is considered appropriate within its context~\cite{privacy-in-context}. 
%
%Throughout the paper, we refer  as \term{``data flow''} to the tuple \dataflowtuple, consistently with the 
Inspired by the framework of contextual integrity~\cite{privacy-in-context}, we also seek to characterize whether the data flows are appropriate or not within their context. More specifically, our notion of context includes: {\em consistency}, \ie whether actual data flows extracted from network traffic agree  with the corresponding statements made in the privacy policy; {\em purpose}, extracted from privacy policies and confirmed by destination domains (\eg whether they are ATS); and other information (\eg ``notice and consent'').  
%We then extract, characterize, and compare data flows from two complementary points of view: (1) the \emph{actual} behavior exhibited in the \emph{network traffic} generated by a VR app and platform, and (2) the \emph{declared} behavior in the \emph{privacy policy} of the VR app and platform. 
Our methodology and system, \tool{}, 
is depicted on \figref{}~\ref{fig:our-work}. Next we summarize our methodology and findings.

\vspace{5pt}
\myparagraph{Network traffic: methodology and findings.} 
%In \secref{}~\ref{sec:network-traffic-analysis}, 
\minorrevision{We were able to explore 140 popular, paid and free, \oculusvr{} apps; and then capture, decrypt, and analyze the network traffic they generate in order to assess their practices with respect to collection and sharing of personal data on the \oculusvr{} platform.} 
%\rahmadi{We started with 150 popular, paid and free, \oculusvr{} apps, we explored them to generate rich network traffic} \athina{and we were able to inspect and analyze the traffic of 140 of them.}
%We used the best known practices to explore these apps %, enable \tool{}, 
%and generate rich network traffic for 140 of them. %~\cite{varmarken2020tv} and we experimented with the top-150 \oculusvr{} apps.

%
\tool{} collects network traffic without rooting the \device{}, by building on the open-source  AntMonitor~\cite{shuba2016antmonitor}, which we had to modify to work on the Android 10-based Oculus OS. %\footnote{Antmonitor only works on Android 7, an OS that was released in 2016.}. 
\minorrevision{
Furthermore, we successfully addressed new technical challenges for decrypting network traffic on \oculusvr{}. \tool{} combines  dynamic analysis (using} Frida~\cite{frida-tool}) \minorrevision{with binary analysis to find and bypass certificate validation functions, even when the app contains a stripped binary~\cite{Unity-strip}.} This was a  challenge specific to \oculusvr{}: prior work on decrypting network traffic on Android~\cite{shuba2020nomoats,mohajeri2019watching} hooked into standard Android SDK functions and not the ones packaged with Unity and Unreal, which are the basis for game apps.
 %Notably, our pipeline permits for the exercising of apps wirelessly, allowing for free-roaming testing of VR apps.


We extracted and analyzed data flows found in the collected network traffic from the 140 OVR apps, and we made the following observations. 
%
We studied a broad range of 21 data types that are exposed and found that 33 and 70 apps send PII data types (\eg Device ID, User ID, and Android ID) to first-and third-party destinations, respectively (see Table~\ref{tab:pii-summary}). Notably, 58 apps expose VR sensory data (\eg physical movement, play area) to third-parties.
\minorrevision{
We used state-of-the-art \blocklist{s} to identify ATS and discovered that, unlike other popular platforms (\eg{} Android and Smart TVs), \oculusvr{} exposes data primarily to tracking and analytics services, and has a less diverse tracking ecosystem. Notably, the \blocklist{s} identified only 36\% of these exposures. On the other hand, we found no data exposure to advertising services as ads on \oculusvr{} is still in an experimental phase~\cite{oculus-ads}. 
}
%We used state-of-the-art \blocklist{s} to identify ATS and discovered that unlike other popular platforms, such as Android and Smart TVs, (1) \oculusvr{} exposes data primarily to tracking and analytics services, but not to advertising services, and (2) the \blocklist{s} block only 36\% of these exposures. %third party tracking.
%
%A possible explanation is that Facebook keeps all ads on \oculusvr{} within its own ad ecosystem or that the technology to display ads within VR apps are not ready for use. 
%
%Lastly, we found that the \blocklist{s} capture only 36\% of third party data type \term{exposures}.



\myparagraph{Privacy policy: methodology and findings.}
%In \secref{}~\ref{sec:privacy-policy}, 
We provide an NLP-based methodology for analyzing the privacy policies that accompany VR apps. More specifically, \tool{}  maps each data flow (found in the network traffic) to its corresponding  data collection statement (found in the text of the privacy policy), and checks the {\em consistency} of the two. Furthermore, it extracts the {\em purpose} of data flows from the privacy policy, as well as from the ATS analysis of destination domains. Consistency, purpose, and additional information provide {\em context}, in which we can holistically assess the appropriateness of a data flow \cite{privacy-in-context}. Our methodology builds on, combines, and  improves state-of-the-art tools originally developed for mobile apps:  \policylint{}~\cite{andow2019policylint}, \policheck{}~\cite{andow2020actions}, and \polisys{}~\cite{harkous2018polisis}.
We curated VR-specific ontologies for data types and entities, guided by both the network traffic and privacy policies. We also interfaced between different NLP models of \policheck{} and \polisys{} to extract the purpose behind each data flow. 
%are necessary for consistency analysis of network traffic and policies specifically for VR. 
%We also combined all the pieces to include the purpose and characterize for the first time the full context of data flows: \dataflowtuple.

%in conjunction with the app's actual behavior (\ie network traffic) for data-flow-to-policy 
%
%We developed VR-specific ontologies for data types and entities that are necessary for accurate disclosure classification of data flows from VR apps.  
%Furthermore,\tool{} improves the first-party resolution process.
%To the best of our knowledge, this is the first work that performs consistency analysis of network traffic and policies specifically for VR, while prior work focused on mobile \cite{andow2020actions}; \athina{difference X% here}.  % and the first to characterize the full context including 

%Next, we characterize the behavior of VR apps based on data flows.
%
Our network-to-policy consistency analysis revealed that about 70\% of data flows from  VR apps were not disclosed or consistent with their privacy policies\minorrevision{: only 30\% were consistent}. Furthermore, 38 apps did not have privacy policies, including apps from the official Oculus app store. Some app developers also had the tendency to neglect declaring data collected by the platform and third parties.
\minorrevision{We found that by automatically including these other parties' privacy policies in \tool{}'s network-to-policy consistency analysis, 74\% of data flows became consistent.
}
We also found that 69\% of data flows have purposes unrelated to the core functionality \minorrevision{(\eg advertising, marketing campaigns, analytics)}, and only a handful of apps are explicit about notice and consent. 
%\todo{From Hieu: Rah or Hao add (1) positive findings about referencing third/first party privacy policies = good consistency. (2) disclosure findings.}
%\emph{advertising} (32\%) and \emph{analytics} (19\%) are the two main purposes of data flows, whereas only a handful of apps are explicit about notice and consent. % for data collection and sharing. %explicitly ask users to read their privacy policies and give consent for data collection. 
\minorrevision{\tool{}'s implementation and datasets are made available at~\cite{ovrseen-release}.} 
%\athina{[New numbers??]}

%Thus, we had to significantly improve PoliCheck. In addition to extending its synonym list with new terms, we had to substantially modify its entity and data type ontologies (as was also done previously in~\cite{lentzsch2021heyalexa}) to specifically include VR-specific data types. We also performed non VR-specific improvements in other parts of PoliCheck (\eg first-party resolution process). We outline the detail of this improvement process in \secref{}~\ref{sec:improving-policheck}.
%We believe that these can benefit other researchers that plan to use and adapt PoliCheck into other platforms in the future.
%We plan to release our dataset, and the source code of our data collection automation software and the improved PoliCheck.



\mycomment{
In terms of app ecosystem, Oculus is also unique compared to other platforms.
A platform usually has a major official app store that users mainly use (\eg Android has Google Play store, and Amazon's Fire TV has Fire TV app store as their official app stores) and a number of small third-party app stores that are not popular. 
On the contrary, Oculus has an official app store that is closely related to SideQuest, a third-party app store specifically endorsed by Facebook~\cite{oculus-sidequest}---Oculus was a VR company that was bought by Facebook in 2014. Apps available on SideQuest are typically under development---their trial or beta versions are first released on SideQuest to attract users before finally released on the official Oculus app store.
}











\mycomment{
Finally, we evaluated the privacy policies from apps (see \secref{}~\ref{sec:privacy-policy}).
We used PoliCheck~\cite{andow2020actions} to analyze the consistency of a privacy policy against the app's network traffic, and Polisis~\cite{harkous2018polisis} to further analyze parts and \emph{context} (\ie data types, recipient, and collection purposes) of a privacy policy.
We discovered that many apps either do not have privacy policies (including apps from the official Oculus app store), or have poorly-written privacy policies. For instance, app developers tend to neglect declaring data collections performed by the platform and third-party libraries.
}





\mycomment{
First, network traffic decryption is extremely challenging for VR apps (see \secref{}~\ref{sec:data-collection}). 
Most VR apps are developed using third-party frameworks, such as Unity and Unreal~\cite{unity-framework,unreal-framework}. These frameworks typically compile their SDK into stripped binary files to increase performance on a VR device---these apps are usually 3D games that require a lot of processing power and memory.
Thus, the commonly used techniques known by the research community~\cite{shuba2020nomoats,mohajeri2019watching,varmarken2020tv} (\ie bypassing SSL certificate checks and pinning by manipulating the Android SDK library) to decrypt normal Android apps cannot be deployed to decrypt traffic from VR apps.
Thus, our work presents a novel technique, in which we perform binary analysis to find the right functions to manipulate in the stripped binary files to facilitate traffic decryption---a stripped binary file does not contain any symbol table.

Second, PoliCheck~\cite{andow2020actions} cannot be used directly to check privacy policy compliance for VR apps since it was first tailored for checking Android apps (see \secref{}~\ref{sec:privacy-policy}). In addition to extending its synonym list with new terms, we had to significantly modify its entity and data type ontologies (as previously also done in previous work~\cite{lentzsch2021heyalexa}) to particularly include VR-specific data types.
We also improved other aspects of PoliCheck that can support future research on other platforms, \eg we significantly improved its policy pre-processing.

%\myparagraph{Contributions.}
Despite these challenges, our work makes the following contributions:
\begin{itemize}
    \item We perform the first wide-scale systematic study of the privacy aspects of VR apps. We perform our study on the Oculus platform that the research community has been looking into for VR research.
    \item We automate much of our data collection process. Since we still require a human tester for VR apps, we integrate this manual testing seamlessly into our automation pipeline. Our work also highlights the novel technique to decrypt network traffic from VR apps.
    \item We present comprehensive analysis and evaluation of various privacy aspects of VR: ATS ecosystem, PII exposures, and privacy policies of VR apps. Most notably, VR platform data collections include VR-specific data types. We also significantly improved PoliCheck, when adjusting it for VR apps.
\end{itemize}
}


%\figref{}~\ref{fig:our-work} provides an overview of our methodology, \tool{}.
\myparagraph{Overview.} The rest of this paper is structured as follows.
\secref{}~\ref{sec:background} provides background on the \oculusvr{} platform and its data collection practices that motivate our work. 
\secref{}~\ref{sec:network-traffic-analysis} provides the methodology and results for \tool{}'s network traffic  analysis. 
%\secref{}~\ref{sec:dataset} describes our app corpus and datasets.
%\secref{}~\ref{sec:ats-pii-analyses} reports the results of our ATS and PII analyses.
\secref{}~\ref{sec:privacy-policy} provides the methodology and results for \tool{}'s policy analysis, network-to-policy consistency analysis, and purpose extraction.
\minorrevision{\secref{}~\ref{sec:discussion} discusses %and highlights the uniqueness of VR, threats to validity, recommendations, and responses from Oculus and app developers about our findings.
the findings and provides recommendations.}
\secref{}~\ref{sec:related-work} discusses related work.
\secref{}~\ref{sec:limitation-conclusion} concludes the paper. 



%\myparagraph{Challenges.}
%In our data collection and analyses, we encountered 3 main challenges.
%First, we attempt to automate the data collection process as much as possible. However, unlike Android phones whose testing process can be automated simply by emulating sequences of user inputs (\eg button presses)~\cite{li2017droidbot}, a VR device still requires a human tester---emulating a human player playing a VR game is a non-trivial problem. 
%Thus, we only automate the steps that do not require human interaction (\eg app repackaging and network traffic recording) and seamlessly integrate it with the human testing.

%First, network traffic decryption is extremely challenging for VR apps (see \secref{}~\ref{sec:data-collection}). 
%Most VR apps are developed using third-party frameworks, such as Unity and Unreal~\cite{unity-framework,unreal-framework}. These frameworks typically compile their SDK into stripped binary files to increase performance on a VR device---these apps are usually 3D games that require a lot of processing power and memory.
%Thus, the commonly used techniques known by the research community~\cite{shuba2020nomoats,mohajeri2019watching,varmarken2020tv} (\ie bypassing SSL certificate checks and pinning by manipulating the Android SDK library) to decrypt normal Android apps cannot be deployed to decrypt traffic from VR apps.

%Second, PoliCheck~\cite{andow2020actions} cannot be used directly to check privacy policy compliance for VR apps since it was first tailored for checking Android apps (see \secref{}~\ref{sec:privacy-policy}). In addition to extending its synonym list with new terms, we had to significantly modify its entity and data type ontologies (as previously also done in previous work~\cite{lentzsch2021heyalexa}) to particularly include VR-specific data types.
%We also improved other aspects of PoliCheck, \eg privacy policy text pre-processing.


==> VR Project (USENIX Security 2022)/privacy_policy.tex <==
% \begin{figure*}[!htb]
% 	\centering
% 	\includegraphics[width=0.8\textwidth]{images/policheck/data_ontology.pdf}
% 	\caption{\textbf{Modified Data Ontology.} Nodes printed in bold are new nodes added on top of PoliCheck's ontology. Nodes with non-italic labels are leaf nodes, which correspond to data types in data flows.}
% 	\label{fig:data-ontology}
% \end{figure*}

% \begin{figure}[ht!]
% 	\centering
% 	\includegraphics[width=1\columnwidth]{images/policheck/entity_ontology.pdf}
% 	\caption{\textbf{Modified Entity Ontology.} Leaf nodes inherited from PoliCheck's entity ontology are merged in order to save space.}
% 	\label{fig:entity-ontology}
% \end{figure}



\section{\tool{}: Privacy Policy Analysis}
\label{sec:privacy-policy}

In this section, we turn our attention to the intended data collection and sharing practices, as stated in the text privacy policy. % In particular, we obtain and analyze the text of these privacy policies \wrt data collection and sharing statements and purposes. 
For example, from the text {\em ''We may collect your email address and share it for advertising purposes''}, we want to extract the collection statement (``we'', which implies the app's first-party entity; ``collect'' as action; and ``email address'' as data type) and the purpose (``advertising''). In \secref{}~\ref{sec:policheck-polisys}, we present our methodology for extracting data collection statements, and comparing them against data flows found in network traffic for consistency. \tool{} builds and improves on state-of-the-art NLP-based tools: \policheck{}~\cite{andow2020actions} and \policylint{}~\cite{andow2019policylint}, previously developed for mobile apps. In \secref{}~\ref{sec:policy-ontology}, we present our VR-specific ontologies for data types and entities.  % and \polisys{}~\cite{harkous2018polisis}.
%In this section, we describe how we collect and analyze privacy policies to perform
%data-to-flow-consistency analysis , and report our findings. 
%We modified PoliCheck~\cite{andow2020actions} and integrated the improved version into \tool{}.
%Recall that \tool{} integrates PoliCheck~\cite{andow2020actions} and Polisis~\cite{harkous2018polisis} for privacy policy analysis.
%\secref{}~\ref{sec:policheck-improvement} outlines how we developed \tool{}'s VR-specific ontologies to check the consistency of each app's privacy policy with respect to the app's network traffic, while \secref{}~\ref{sec:policheck-results} reports our analysis results.
In \secref{}~\ref{sec:policheck-results}, we report network-to-policy consistency results.
\secref{}~\ref{sec:polisis-context} describes how we interface between the different NLP models of \policheck{} and  \polisys{} to extract the data collection purpose and other context for each data flow. %; this corresponds to  \circled{\textbf{5}} in \figref{}~\ref{fig:our-work}. \athina{shrink}

\myparagraph{Collecting privacy policies.}
For each app in \secref{}~\ref{sec:network-traffic-analysis}, we also collected its privacy policy on the same day that we collected its network traffic. %, as described in \secref{}~\ref{sec:network-traffic-collection}. 
Specifically, we used an automated Selenium~\cite{selenium} script to crawl the webstore and extracted URLs of privacy policies. For apps without a policy listed, we followed the link to the developer's website to find a privacy policy.  We also included eight third-party policies (\eg from Unity, Google), referred to by the apps' policies.
%---we also collected Oculus and third-party privacy policies at around the same time. 
%This ensures that the collected privacy policies reflects the actual data collection practices observed in the corresponding network traffic in \secref{}~\ref{sec:network-traffic-dataset}.

For the top-50 free apps on the Oculus store, we found that only 34 out of the 43 apps have privacy policies.  Surprisingly, for the top-50 paid apps, we found that only 39 out of 49 apps have privacy policies.
For the top-50 apps on SideQuest, we found that only 29 out of 48 apps have privacy policies.
Overall, among apps in our corpus, we found that only 102 (out of 140) apps provide valid English privacy policies.   We treated the remaining apps as having empty privacy policies, ultimately leading \tool{} to classify their data flows as omitted disclosures.
\vspace{-5pt}
%Our \netdataset{} consists of \tcpflowtotal{} TCP flows from 140 apps (see \tabref{}~\ref{tab:dataset-summary}). Data type exposures were found in 1,623 TCP flows and then converted into \dataflowtotal{} unique data flows for consistency analysis.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsection{\tool{} Privacy Policy Analyzer}
\subsection{Network-to-Policy Consistency}
\label{sec:policheck-improvement}

Our goal is to analyze text in the app's privacy policy, extract statements about data collection (and sharing), and compare them against the actual data flows found in network traffic. 

\subsubsection{Consistency Analysis System}
\label{sec:policheck-polisys}

%``If you register for our cloud services, we will collect your email address and share it for advertising purposes''
\tool{} builds on state-of-the-art tools: \policylint{}~\cite{andow2019policylint} and \policheck{}~\cite{andow2020actions}.  \policylint{}~\cite{andow2019policylint} provides an NLP pipeline that takes a sentence as input. For example, it takes the sentence {\em ``We may collect your email address and share it for advertising purposes''}, and extracts the collection statement ``(entity: \emph{we}, action: \emph{collect}, data type: \emph{email address})''.
More generally, \policylint{} takes the app's privacy policy text, parses sentences and performs standard NLP processing, and eventually extracts data collection statements defined as the tuple $P=$\polichecktuple{}, where \textit{app} is the sender and \textit{entity} is the recipient performing an \textit{action} (collect or not collect) on the \textit{data type}.
\policheck{}~\cite{andow2020actions}  takes the app's data flows (extracted from the network traffic and defined as $F=$\policheckdataflow{}) and compares it against the stated $P$ for consistency. 

\policheck{} classifies the disclosure of $F$ as {\em clear} (if the data flow exactly matches a collection statement), {\em vague} (if the data flow  matches a collection statement in broader terms), {\em omitted} (if there is no collection statement corresponding to the data flow), {\em ambiguous} (if there are contradicting collection statements about a data flow), or {\em incorrect} (if there is a data flow for which the collection statement states otherwise). 
Following \policheck{}'s terminology~\cite{andow2020actions}, we further group these five types of disclosures into  two groups: \emph{consistent} (clear and vague disclosures) and \emph{inconsistent} (omitted, ambiguous, and incorrect) disclosures. 
The idea is that for consistent disclosures,  there is a statement in the policy that matches the data type and entity, either clearly or vaguely.
\minorrevision{
 \tabref{}~\ref{tab:policy-sentence-vs-data-flow} provides real examples of data collection disclosures extracted from VR apps that we analyzed.
}
%


\begin{table*}[t!]
	\tabletextsize
	\centering
	\minorrevision{
	\begin{tabularx}{\linewidth}{c | p{15mm} p{55mm} p{50mm} p{35mm}}
	    \toprule
		\multicolumn{2}{c}{\textbf{Disclosure Type}} &  \textbf{Privacy Policy Text} & 
		\textbf{Action : Data Collection Statement (P)} & \textbf{Data Flow (F)} 
		\\
		%\midrule
		%\multicolumn{4}{c}{\textbf{Consistent Disclosures}}\\
		\midrule
		\multirow{2}{*}{\rotatebox[origin=c]{90}{\textbf{Consistent}}}
		%For example, we collect information like web requests, the data sent in response to such requests, the Internet Protocol address, the browser type, the browser language, and a timestamp for the request.
		& Clear & ``For example, we collect information ..., and \textit{a timestamp for the request}.'' & \emph{collect : $\langle$com.cvr.terminus, usage time, we$\rangle$} & \emph{$\langle$usage time, we$\rangle$} \\
		\cline{2-5}
		%We will share your information (in some cases personal information) with third-parties, that is parties other than Home Net Games, in the following circumstances
	    & Vague & ``We will share \emph{your information (in some cases} & \emph{collect : $\langle$com.HomeNetGames.WW1oculus,} & \emph{$\langle$serial number, oculus$\rangle$}\\
	    & & \emph{personal information)} with third-parties, ...'' & \emph{pii, third party$\rangle$} & \emph{$\langle$android id, oculus$\rangle$}\\
	    \midrule
	    %\multicolumn{4}{c}{\textbf{Inconsistent Disclosures}}\\
	    & Omitted & - & \emph{collect : $\langle$com.kluge.SynthRiders, -, -$\rangle$} & \emph{$\langle$system version, oculus$\rangle$}\\
	    & & & & \emph{$\langle$sdk version, oculus$\rangle$}\\
	    & & & & \emph{$\langle$hardware information, oculus$\rangle$}\\
	    \cline{2-5}
	    % Except as set forth in this Privacy Policy or as specifically agreed to by you, Skydance will not disclose any Personally Identifiable Information to third parties we collect from you on the Website.||your Personally Identifiable Information will be disclosed to such third parties and all information you disclose will be subject to the privacy policy and practices of such third parties.
	    \multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{Inconsistent}}}
	    & Ambiguous & ``..., Skydance \emph{will not disclose any Personally} & \emph{collect : $\langle$com.SDI.TWD, pii, third party$\rangle$} & \emph{$\langle$serial number, oculus$\rangle$}\\
	    & & \emph{Identifiable Information to third parties} ... & & \emph{$\langle$android id, oculus$\rangle$}\\
	    & & your \emph{Personally Identifiable Information will be disclosed to such third parties} and ...'' & & \\
	    \cline{2-5}
	    & Incorrect & ``We \emph{do not share our customer's personal in-} & \emph{not\_collect : $\langle$com.downpourinteractive.} & \emph{$\langle$device id, unity$\rangle$}\\
	    & & \emph{formation with unaffiliated third parties} ...'' & \emph{onward, pii, third party$\rangle$} & \emph{$\langle$user id, oculus$\rangle$}\\
	    \bottomrule
	\end{tabularx}
    }
	\vspace{-5pt}
	\caption{\minorrevision{\textbf{Examples to illustrate the types of disclosures identified by \policheck{}.} 
A {\em data collection statement (P)} is extracted from the privacy policy text and is defined as the tuple $P=$\polichecktuple{}. {\em A data flow (F)} is extracted from the network traffic and is defined as $F=$\policheckdataflow{}. During the consistency analysis, each $P$ can be mapped to zero, one, or more $F$.}}
	\label{tab:policy-sentence-vs-data-flow}
	\vspace{-10pt}
\end{table*}




Consistency analysis relies on pre-built ontologies and synonym lists used to match (i) the data type and destination that appear in each $F$ with (ii) any instance of $P$ that discloses the same (or a broader) data type and destination\footnote{For example (see \figref{}~\ref{fig:data-ontology}), ``email address'' is a special case of ``contact info'' and, eventually, of ``pii''. There is a clear disclosure \wrt data type if the ``email address'' is found in a data flow and a collection statement. A vague disclosure is declared if the ``email address'' is found in a data flow and a collection statement that uses the term ``pii'' in the privacy policy. An omitted disclosure means that ``email address'' is found in a data flow, but there is no mention of it (or any of its broader terms) in the privacy policy.}.
%Clear and vague disclosures are referred to together as {\em consistent} since there is a statement in the policy that matches the data type and entity either clearly or vaguely. The remaining three labels are referred to together as {\em inconsistent}.
 \tool{}'s adaptation of ontologies specifically for VR is described in  \secref{}~\ref{sec:policy-ontology}. 
% 
We also improved several aspects of \policheck{}, as described in detail in \appdx{\appref{}~\ref{app:other-policheck-improvements}}.
First, we added a feature  to include a third-party privacy policy for analysis if it is mentioned in the app's policy. We found that 30\% (31/102) of our apps' privacy policies reference third-party privacy policies, and the original \policheck{} would mislabel third-party data flows from these apps as omitted. Second, we added a feature to more accurately resolve first-party entity names. Previously, only first-person pronouns (\eg ``we'') were used to indicate a first-party reference, while some privacy policies use company and app names in first-party references. The original \policheck{} would incorrectly recognize these first-party references as third-party entities for 16\% (16/102) of our apps' privacy policies. 
 

\mycomment{
To facilitate this analysis, PoliCheck uses pre-built ontologies and a synonym list
(that contains synonyms for every term that appears in the ontologies)
to match data types and destinations (\ie entities) appearing in privacy policy texts against those appearing in network traffic.
More specifically, PoliCheck performs the following steps:
\squishcount
    \item \textit{Pattern extraction:} PoliCheck takes privacy policy texts as input, and extract tuple $P=<\text{app name}, \text{entity}, \text{action}, \text{data type}>$ from each policy statement---action is either \textit{collect} or \textit{not collect}.
    \item \textit{Flow labeling:} we extract data flows, each in the form of tuple $F=<\text{app name}, \text{data type}, \text{entity}>$, from the network traffic. 
    \item \textit{Consistency analysis:} for each $F$, PoliCheck searches $P$ that represents the policy statement that discloses $F$.
    PoliCheck uses the ontologies and synonym lists to match the data types and entities that appear in each $F$ with any instance of $P$ that discloses similar data types and entities. 
    \item \textit{Disclosure classification:} PoliCheck classifies each $F$ as either
    clear, vague, omitted, ambiguous, or incorrect disclosure.
\countend
}

\mycomment{
\begin{figure}[t!]
    \centering
        \includegraphics[width=0.98\columnwidth]{images/policheck/data_ontology2.pdf}
    \caption{\textbf{Data Ontology for VR.} Nodes in bold are newly added to the original data ontology. %Nodes with non-italic labels are leaf nodes, correspond to data types in data flows.
    }
    \label{fig:data-ontology}
    \vspace{-10pt}
\end{figure}
}


%\mycomment{
\begin{figure*}
    \centering
    \vspace{-5pt}
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/policheck/data_ontology2.pdf}
        \caption{Data Ontology}
        \label{fig:data-ontology}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.39\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/policheck/entity_ontology2.pdf}
        \caption{\minorrevision{Entity Ontology}}
        \label{fig:entity-ontology}
    \end{subfigure}
    \vspace{-8pt}
    \caption{\minorrevision{\textbf{Ontologies for VR data flows.} Please recall that each data flow, {\em F}, is defined as $F=$\policheckdataflow{}. We started from the \policheck{} ontologies, originally developed for Android (printed in gray). First, we eliminated nodes that did not appear in our VR network traffic and privacy policies. Then, we added new leaf nodes (printed in black) based on new data types found in the VR network traffic and/or privacy policies text. Finally, we defined additional non-leaf nodes, such as  ``biometric info'' and ''api'', in the resulting VR data and entity ontologies.}}
    %Non-leaf nodes are printed in italic.\athina{[why?]}}
    %{\bf [AM: Check correctness of above text. Why do we need italic in non-leaf nodes?they are already distinct by being non-leaf.]}} 
    %Nodes with non-italic labels are leaf nodes, which correspond to data types and entity names in data flows. 
    \vspace{-1em}
    \label{fig:ontologies}
\end{figure*}
%}




\subsubsection{Building Ontologies for VR}
\label{sec:policy-ontology}




Ontologies are used to represent subsumptive relationships between terms: a link from term \textit{A} to term \textit{B} indicates that \textit{A} is a broader term (\textit{hypernym}) that subsumes \textit{B}.  
There are two ontologies, namely data and entity ontologies: the data ontology maps data types and entity ontology maps destination entities. 
 Since \policheck{} was originally designed for Android mobile app's privacy policies, it is important to adapt the ontologies to include data types and destinations specific to VR's privacy policies and  actual data flows.
%\mysubparagraph{Data Ontology.}



\myparagraph{VR data ontology.} 
\figref{}~\ref{fig:data-ontology} shows the data ontology we developed for VR apps.
%\figref{}~\ref{fig:data-ontology} shows PoliCheck's data ontology that has been adapted for VR apps.
Leaf nodes correspond to all 21 data types found in the network traffic and listed in \tabref{}~\ref{tab:pii-summary}. Non-leaf nodes are broader terms extracted from privacy policies and may subsume more specific data types, \eg ``device identifier'' is a non-leaf node that subsumes ``android id''. We built a VR data ontology, starting from  the original Android data ontology, in a few steps as follows.
First, we cleaned up the original data ontology by removing data types that do not exist on \oculusvr{} (\eg ``IMEI'', ``SIM serial number'', \etc). We also merged similar terms (\eg ``account information'' and ``registration information'') to make the structure clearer. 
%{\cuihao (PoliCheck's ontologies have some redundant nodes inherited from PolicyLint's auto-generated ontologies. \eg \textit{account information} and \textit{registration information})}
\minorrevision{
Next, we used PoliCheck to parse privacy policies from VR apps.
When PoliCheck parses the sentences in a privacy policy, it extracts terms and tries to match them with the nodes in the data ontology and the synonym list. If PoliCheck does not find a match for the term, it will save it in a log file.
We inspected each term from this log file, and added it either as a new node in the data ontology or as a synonym to an existing term in the synonym list.
}
%Specifically, we ran PoliCheck against privacy policy texts from VR apps and checked log files to identify new terms that refer to data types. We manually add them to the ontology.
Finally, we added new terms for data types identified in network traffic (see \secref{}~\ref{sec:pii-exposures}) as leaf nodes in the ontology. 
Most notably, we added VR-specific data types (see VR Sensory Data category shown in \tabref{}~\ref{tab:pii-summary}): ``biometric info'' and ``environment info''. The term ``biometric info'' includes physical characteristics of human body (\eg height, weight, voice, \etc); we found some VR apps that collect user's ``pupillary distance'' information. The term ``environment information'' includes VR-specific sensory information that describes the physical environment; we found some VR apps that collect user's ``play area'' and ``movement''.
%In addition to data types found in PII analyses, we found a few new vague data-type terms that were not in PoliCheck's ontology:
%\begin{itemize}
%    \item \textit{biometric information}: This includes physical characteristics of human body from body height and weight to voice and fingerprint. In practice, we found that some apps sent \textit{pupillary distance} of players, which can be seen as biometric information.
%    \item \textit{environment information}: VR devices are rich of sensors that can be used to measure the physical environment. We found that some apps sent \textit{play area} and \textit{movement} of users, which may be linked to this data-type terms.
%    \item \textit{fingerprint}, \textit{software information}, \textit{hardware information}...: These are not likely unique to the VR platform. PoliCheck's data ontology doesn't have these nodes because the authors didn't consider them in data-flow-to-policy consistency analysis. However, a combination of these data can be used in fingerprinting. We added them to the ontology to expand the scope of our analysis.
%\end{itemize}
\tabref{}~\ref{tab:new-ontology-summary} shows the summary of the new VR data ontology. It consists of 63 nodes: 39 nodes are new in \tool{}'s data ontology.
%\figref{}~\ref{fig:data-ontology} shows our VR data ontology.
%\figref{}~\ref{fig:data-ontology} shows the full data ontology, but omitting \athina{[why?]} leaf nodes that were found in privacy policies but did not appear in our network traffic dataset (\eg ``MAC address'' and ``phone number'').
%Even though these data types appear in privacy policies, removing them does not affect data-flow-to-policy consistency as long as they are not found in any data flows.
Overall, the original Android data ontology was used to track 12 data types (\ie 12 leaf nodes)~\cite{andow2020actions}, whereas our VR data ontology is used to track 21 data types (\ie 21 leaf nodes) appearing in the network traffic (see~\tabref{}~\ref{tab:pii-summary} and \figref{}~\ref{fig:data-ontology}).




%\mysubparagraph{Entity Ontology.} 
\myparagraph{VR entity ontology.} 
Entities are names of companies and other organizations which refer to destinations. 
\minorrevision{
We use a list of domain-to-entity mappings to determine which entity  each domain belongs to (see \appdx{\appref{}~\ref{app:other-policheck-improvements}})---domain extraction and categorization as either first-, third-, or platform-party are described in detail in \secref{}~\ref{sec:labeling-data-flow}.} 
We modified the Android entity ontology to adapt it to VR as follows: (1) 
we pruned entities that were not found in privacy policies of VR apps or in our network traffic dataset, and (2) we added new entities found in both sources.
\tabref{}~\ref{tab:new-ontology-summary} summarizes the new entity ontology. It consists of 64 nodes: 21 nodes are new in \tool{}'s entity ontology.
%---this is much smaller than the original entity ontology because our dataset contains fewer apps.
\figref{}~\ref{fig:entity-ontology} shows our VR entity ontology, in which we added two new non-leaf nodes: ``platform provider'' (which includes online distribution platforms or app stores that support the distribution of VR apps)  and ``api'' (which refers to various third-party APIs and services that do not belong to existing entities).
We identified 16 new entities that were not included in the original entity ontology. We visited the websites of those new entities and found that: three are platform providers, four are analytic providers, and 12 are service providers; these become the leaf nodes of ``api''.
We also added a new leaf node called ``others'' to cover a few data flows, whose destinations cannot be determined from the IP address or domain name.

\begin{table}[t!]
%	\tabletextsize
	\centering
	\begin{tabularx}{\linewidth}{X  r  r}
	    \toprule
		\textbf{Platform} & \textbf{Data Ontology} & \textbf{Entity Ontology}
		\\
		\midrule
		%Android ~\cite{andow2020actions} & 38 nodes / 62 edges & 209 nodes / 236 edges  \\
		Android ~\cite{andow2020actions} & 38 nodes & 209 nodes \\
		%Oculus  & 63 nodes / 77 edges & 64 nodes / 76 edges  \\
		\oculusvr{} (\tool) & 63 nodes & 64 nodes \\
		\midrule
		\rowcolor{brandeisblue!10}
		\textit{New nodes in \oculusvr{}} & 39 nodes            &  21 nodes  \\
	    \bottomrule
	\end{tabularx}
	\caption{Comparison of \policheck{} and \tool{} Ontologies. Nodes include leaf nodes (21 data types %[coincidence?]
	 and 16 entities) and non-leaf nodes (see \figref{}~\ref{fig:ontologies}). }
	\label{tab:new-ontology-summary}
	\vspace{-12pt}
\end{table}


\myparagraph{Summary.}
Building VR ontologies has been non-trivial.
We had to examine a list of more than 500 new terms and phrases that were not part of the original ontologies.
Next, we had to decide whether to add a term into the ontology as a new node, or as a synonym to an existing node.
In the meantime, we had to remove certain nodes irrelevant to VR and merge others because the original Android ontologies were partially machine-generated and not carefully curated.
%We also shared our methodology to adapt the original ontologies into the VR domain---this is useful for adapting the system for other ecosystems.
%Thus, these improvements are meant not only to adapt PoliCheck for privacy policies of VR apps, but also prepare PoliCheck to better support future research.


\begin{figure*}[!t]
	\centering
	\vspace{-10pt}
	\includegraphics[width=0.9\textwidth]{images/policheck/heatmap_all.pdf}
	\vspace{-1em}
	\caption{\textbf{Summary of network-to-policy consistency analysis results.} Columns whose labels are in parentheses provide aggregate values: \eg column ``(platform)'' aggregates the columns ``oculus'' and ``facebook''; column ``(other 3rd parties)'' aggregates the subsequent columns. The numbers count data flows; each data flow is defined as \dataflowtuple{}).}
	%(entities connected by less than 2 apps are not shown)}
	\label{fig:heatmap-all}
	\vspace{-10pt}
\end{figure*}




\subsubsection{Network-to-Policy Consistency Results}

\label{sec:policheck-results}
%We ran our improved version of PoliCheck with adapted ontologies on our dataset.
We ran \tool{}'s privacy policy analyzer to perform network-to-policy consistency analysis. Please recall that we extracted \dataflowtotal{} data flows from 140 apps (see \secref{}~\ref{sec:labeling-data-flow}).  
%Following \policheck{}'s terminology~\cite{andow2020actions}, we further groups the five types of disclosures into  two groups: \emph{consistent} (clear and vague disclosures) and \emph{inconsistent} (omitted, ambiguous, and incorrect) disclosures.

% Recall that PoliCheck classifies each data flow based on 5 disclosure types. We adopt terminologies from ~\cite{andow2020actions} and consider clear and vague disclosures as \emph{consistent} disclosures; and omitted, ambiguous, and incorrect disclosures as \emph{inconsistent} disclosures.



\myparagraph{\oculusvr{} data flow  consistency.}
%\emph{In general, our main finding is that apps in our corpus, despite being top VR apps, do not properly disclose their data collection practices.}
In total, 68\% (776/1,135) data flows are classified as inconsistent disclosures.  The large majority of them 97\% (752/776) are omitted disclosures, which are not declared at all in the apps' respective privacy policies.
\figref{}~\ref{fig:heatmap-all} presents the data-flow-to-policy consistency analysis results. Out of 93 apps which expose data types, 82 apps have at least one inconsistent data flows. 
%
Among the remaining 32\% (359/1,135) consistent data flows, 86\% (309/359) are classified as vague disclosures. They are declared in vague terms in the privacy policies (\eg the app's data flows contain the data type ``email address'', whereas its privacy policy only declares that the app collects ``personal information''). Clear disclosures are found in only 16 apps.

%Overall, only 31.6\% (359/1,135) data flows are classified as consistent disclosures---86.1\% (309/359) of them are classified as vague disclosures. Thus, most data flows that \tool{} classifies as having consistent disclosures are declared in vague terms in the privacy policies (\eg the privacy policy declares that the app collects ``personal information'', whereas the app's data flows contain ``person name''). %\todo{\hieu{Need a sentence on the percentage of consistent disclosures.}}
%In turn, 68.4\% (776/1,135) data flows are classified as inconsistent disclosures.
%Among the inconsistent disclosures, 96.9\% (752/776) are omitted disclosures---these are not declared at all in the apps' respective privacy policies.

% \begin{itemize}
%     \item Stats of apps adhering to policy? Third-party store apps most likely do not have privacy policy at all. SideQuest mostly provides links to the app developer's website or blog. Apps typically have their privacy policy texts if they have been made available on Oculus Store's app lab, which is a section on the store that contains apps that are under development.
%     \item Do direct comparison to~\cite{andow2020actions}: Figure 2, 3, 6, 7, 8 (Facebook mobile app data).
%     \todo{comparison to mobile apps: mimic Fig. 8 in PoliCheck; different ontologies}
%     \item Make recommendations to improve Apps or privacy policies.
% \end{itemize}

\begin{figure}[t!]
    \centering
    %\vspace{-5pt}
    \begin{subfigure}[t!]{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/policheck/bar_dtype_5types.pdf}
        \vspace{-2.5em}
        \caption{}
        \label{fig:policheck-bar-dtype-5types}
    \end{subfigure}
    \hfill\\
    \begin{subfigure}[t!]{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/policheck/bar_entity_5types.pdf}
        \vspace{-2.5em}
        \caption{}
        \label{fig:policheck-bar-entity-5types}
    \end{subfigure}
    \vspace{-5pt}
    \caption{Network-to-policy consistency analysis results aggregated by (a) data types, and (b) destination entities.}
    \label{fig:flow-to-policy-consistency-analysis}
    \vspace{-10pt}
\end{figure}


\mycomment{
\begin{figure}[ht!]
	\centering
	\includegraphics[width=1\columnwidth]{images/policheck/bar_dtype_5types.pdf}
	\caption{\term{Network}-to-policy consistency analysis results aggregated by data types.}
	\label{fig:policheck-bar-dtype-5types}
\end{figure}

\begin{figure}[ht!]
	\centering
	\includegraphics[width=1\columnwidth]{images/policheck/bar_entity_5types.pdf}
	\caption{\term{Network}-to-policy consistency analysis results aggregated by destination entities.}
	%(entities connected by less than 2 apps are not shown).}
	\label{fig:policheck-bar-entity-5types}
\end{figure}

\begin{figure}[ht!]
	\centering
	\includegraphics[width=1\columnwidth]{images/policheck/bar_entity_cmp.pdf}
	\caption{\textbf{Comparisons of \term{network}-to-policy consistency analysis results.} In this graph we compare the results from including Unity and Oculus privacy policies by default and previous results. Previous results are shown by the (rasterized) top bars.}
	\label{fig:policheck-bar-entity-alt}
\end{figure}
}

\vspace{-5pt}
\myparagraph{Data type consistency.} 
%\emph{Our main finding here is that app developers tend to neglect declaring the collection of certain data types in their apps' privacy policies. We suspect the developers deem that collecting these data types is necessary by default to provide the core functionality for their apps.}
%VR Sensory Data and \term{Fingerprinting} fare the worst with only 17.8\% (18/101) and 25.4\% (199/784) of data flows classified as consistent disclosures, respectively.
\figref{}~\ref{fig:policheck-bar-dtype-5types} reports network-to-policy consistency analysis results by data types---recall that in \secref{}~\ref{sec:labeling-data-flow} we introduced all the exposed data types into three categories: \textit{PII}, \textit{Fingerprint}, and \textit{VR Sensory Data}.
The PII category contributes to 22\% (250/1,135) of all data flows.
Among the three categories, PII has the best consistency: 57\% (142/250) data flows in this category are classified as consistent disclosures.
These data types are well understood and also treated as PII in other platforms. 
On Android~\cite{andow2020actions}, it is reported that 59\% of PII flows were consistent---this is similar to our observation on \oculusvr{}.
The Fingerprint category constitutes 69\% (784/1,135) of all data flows: around 25\% (199/784) of data flows in this category are classified as consistent disclosures. 
The VR Sensory Data category constitutes around 9\% (101/1,135) of all data flows---this category is unique to the VR platform. Only 18\% (18/101) data flows of this category are consistent---this indicates that the collection of data types in this category is not properly disclosed in privacy policies.
%In summary, our results indicate that app developers tend to neglect declaring the collection of these data types in their apps' privacy policies. We suspect the developers deem that collecting these data types is necessary by default to provide the core functionality for their apps.

% Hao's note:
% PII: grep -P '^(user id|device id|android id|serial number|person name|email address|geographical)'
% FINGERPRINT: grep -Pv '^(user id|device id|android id|serial number|person name|email address|geographical|vr |flowData)'
% VR: grep -P '^(vr )'

\mycomment{
\myparagraph{PII} PII category, accounting for 22.0\% of data-flow tuples, has the best consistency among three categories, in which 56.8\% (142/250) data-flow tuples are consistent.

These data types are generally well-defined and also treated as personal identifiable information in other platforms. Most of them were also the data types being analyzed in previous works. On Android platform \cite{andow2020actions}, 58.8\% (26,851/45,631 {\cuihao see PoliCheck Table 3}) of PII flows were consistent, which is similar to our observation in the Oculus platform.

\myparagraph{VR sensory data} This category accounts for only 8.90\% (101/1,135) of all data-flow tuples, but the category is unique to the VR platform. Only 14.9\% (15/101) data-flow tuples of this category are consistent, which is far below the average.

The low consistency rate is possibly because many apps treat these data as necessities to provide the core VR functionality so they tend not to explicitly disclose these data types. For example, many privacy policies have vague disclosure like \textit{We collect personal information if it is necessary to provide you the service...}. While this kind of sentences might be used by developers to refer to sensory data in VR apps, it is hard to treat them as effective disclosures.

It is worth noting that most flows of VR sensory data went to Unity (91.1\%, 92/101). Unity may be a third-party data processor of these data. {\cuihao(What is the role of Unity? Why it receives lots of sensory data?)} However, in the later part we will see most apps did poorly in disclosing third-party flows. This is another reason for the low consistency rate of VR sensory data.

\myparagraph{Fingerprint} Fingerprint is the largest category, accounting for 69.1\% (784/1,135) of data-flow tuples. 24.6\% (193/784) of them are consistent. These data types are generally not seen as sensitive information but a combination of them can be used for device fingerprinting. {\cuihao(Cite a paper on fingerprinting. And what does GDPR/CCPA say about this?)}

We suspect that it is possibly because many apps treat these data as necessities to provide the core VR functionality so they tend not to explicitly disclose these data types. For example, many privacy policies have vague disclosure like \textit{We collect personal information if it is necessary to provide you the service...}. While this kind of sentences might be used by developers to refer to sensory data in VR apps, it is hard to treat them as effective disclosures.

It is worth noting that most flows of VR sensory data went to Unity (91.1\%, 92/101). Unity may be a third-party data processor of these data. {\cuihao(What is the role of Unity? Why it receives lots of sensory data?)} However, in the later part we will see most apps did poorly in disclosing third-party flows. This is another reason for the low consistency rate of VR sensory data.
}

%\subsubsection{Entity consistency}
\myparagraph{Entity consistency.}
%\emph{Our main finding here is that apps' privacy policies do not disclose third-party data flows as properly as they do for first-party data flows.}
\figref{}~\ref{fig:policheck-bar-entity-5types} reports our network-to-policy consistency results, by entities.
Only 29\% (298/1,022) of third-party and platform data flows are classified as consistent disclosures.
First-party data flows constitute 10\% (113/1,135) of all data flows: 54\% (61/113) of these first-party data flows are classified as consistent disclosures.
\minorrevision{
Thus, 69\% (785/1,135) of all data flows are classified as inconsistent disclosures.} 
%and only 31\% (350/1,135) are classified as consistent disclosures.
Third-party and platform data flows constitute 90\% (1,022/1,135) of all data flows---surprisingly, only 29\% (298/1,022) of these third-party and platform data flows are classified as consistent disclosures.

Unity is the most popular third-party entity, with   66\% (746/1,135) of all data flows. Only 31\% (232/746) of these Unity data flows are classified as consistent, while the majority (69\%) are classified as inconsistent disclosures. 
Platform (\ie Oculus and Facebook) data flows account for 11\% (122/1,135) of all data flows; only 28\% (34/122) of them are classified as consistent disclosures. 
Other less prevalent entities account only around 14\% (154/1,135) of all data flows.

%\vspace{-2pt}
\myparagraph{Referencing Oculus and Unity privacy policies.}
%\emph{Our main finding here is that both Unity and Oculus privacy policies are well-written.In fact, we found that these 2 privacy policies are among the most detailed and clearest ones.}
Privacy policies can link to each other. For instance, when using \device{}, users should be expected to consent %\footnote{This is the case during the creation of a Facebook account.} 
to the Oculus privacy policy (for \oculusvr{}). Likewise, when app developers utilize a third party engine (\eg Unity) their privacy policies should  include the Unity privacy policy. To the best of our knowledge, this aspect has not been considered in prior work~\cite{zimmeck2017automated,andow2020actions,lentzsch2021heyalexa}.

Interestingly, when we included the Oculus and Unity privacy policies (when applicable) in addition to the app's own privacy policy, we found that the majority of platform (116/122 or 96\%) and Unity (725/746 or 97\%) data flows get classified as consistent disclosures. 
\minorrevision{
Thus, 74\% (841/1,135) of all data flows get classified as consistent disclosures.}
%
%We explore this notion by including the Oculus privacy policy for all apps and Unity privacy policy for all Unity-made apps. 
%First, the Oculus privacy policy clearly lists the categories of information they collect (\eg ``Environmental, Dimensions and Movement Data'', ``Technical System Information'', \etc) and examples of data types they refer to (\eg ``Technical System Information'' includes ``user ID'', ``device ID'', \etc).
%
%We suspected that a huge number of Unity and platform data flows are classified as inconsistent disclosures because apps' privacy policies usually do not refer to Unity and Oculus privacy policies.
%Thus, we experimented more with the 2 privacy policies.
%In this experiment, we included Oculus privacy policy for all apps and Unity privacy policy for apps developed using the Unity framework.
\figref{}~\ref{fig:policheck-bar-entity-alt} shows the comparison of the results from this new experiment  with the previous results shown in \figref{}~\ref{fig:policheck-bar-entity-5types}. 
 These show that data flows are properly disclosed in Unity and Oculus privacy policies even though the app developers' privacy policies usually do not refer to these two important privacy policies.
Furthermore, we noticed that the Oculus and Unity privacy policies are well-written and clearly disclose collected data types. 
As discussed in \cite{andow2020actions}, developers may be unaware of their responsibility to disclose third-party data collections, or they may not know exactly how third-party SDKs in their apps collect data from users. This is a recommendation for future improvement.
%%
%We note that this is the ideal case where app privacy policies link to the appropriate privacy policies. 

%For both app stores, we observed similar trends and characteristics already discussed in this section.
%Most notably, the absence of privacy policies of many apps (including paid apps from the official Oculus app store) contribute significantly to the prevalence of inconsistent (\ie omitted) disclosures.
%In the absence of an app's privacy policy, we ran PoliCheck with an empty text file as the app's ``privacy policy''---thus, PoliCheck considers that the disclosures of all data flows from the app are ``omitted''. 

\begin{figure}[t]
	\centering
	\includegraphics[width=0.85\columnwidth]{images/policheck/bar_entity_cmp.pdf}
	\vspace{-15pt}
	\caption{\textbf{Referencing Oculus and Unity privacy policies.} Comparing the results from the ideal case (including Unity and Oculus privacy policies by default) and the previous actual results (only including the app's privacy policy and any third-party privacy policies linked explicitly therein).}
	\label{fig:policheck-bar-entity-alt}
     \vspace{-5pt} %% never -15! it is visible
\end{figure}

\mycomment{
\myparagraph{\minorrevision{Validation of PoliCheck Results.}}
%\myparagraph{\rahmadi{\policheck{} Validation.}}
\minorrevision{Following the same methodology as the \policheck{} paper \cite{andow2020actions}, we randomly sampled \athina{10 out of 102 apps} with privacy policies and we manually checked their data flows and corresponding collection statements for consistency. Three authors independently checked and agreed on the classification of each data flow. We found the following.}
%\athina{[\bf [AM: can we put the table with the per-class results in the appendix? Like we did for Polisys in Table 7?]}

%\todo{Rahmadi: Hi Athina, I computed the ground truths as it is needed to compute the macro-averaged stuff here; and I had to fix a few results so we ended up now having better results, e.g., micro-averaged precision is now 93.3\%, not 87\% as before; I will work with Hao when he is back to double-confirm.}
\minorrevision{
For {\em binary classification} (\ie to consistent \vs{} inconsistent disclosures), we obtained 94.8\% precision, 100.0\% recall, and 97.3\% F1-score.
For {\em multi-class classification} (\ie we followed \policheck{} to manually validate consistent, omitted and incorrect disclosures), one can assess the micro-averaged or macro-averaged precision, recall, and F1-score\athina{~\cite{macro-vs-micro}}. \athina{The micro-average metrics are more appropriate for imbalanced datasets, and they were used in the \policheck{} paper for Android apps~\cite{andow2020actions} and in another study that applied \policheck{} to Alexa skills~\cite{lentzsch2021heyalexa}.} We found the micro-averaged precision, recall, and F1-score, to be 96.7\%\footnote{\minorrevision{In multi-class classification, every misclassification is a false positive for one class and a false negative for other classes; thus, micro-averaged precision, recall, and F1-score are all the same. Micro-averaged metrics are used to evaluate multi-class classification on imbalanced datasets.}}. This is higher than the corresponding number in~\cite{andow2020actions, lentzsch2021heyalexa}:
both reported 90.8\% precision and 83.3\% precision respectively. For completeness, we also computed the {\em macro-average}, \ie  averaged over all classes,} for multi-class classification and found 
%\athina{{\bf [AM: add citation]}}}
 the macro-averaged precision, recall, and F1-score to be 98.3\%, 97.2\%, and 97.6\% respectively (\appdx{see~\tabref{}~\ref{tab:policheck-eval})}. 
\footnote{However, the precision, recall, and F1-score are lower, when \tool{} has to distinguish between clear and vague disclosures. Our manual validation shows 22.5\% vague disclosures were actually clearly disclosed. This is because \tool{}'s privacy policy analyzer inherits \minorrevision{the limitations of \policheck{}'s NLP model (built on top of \policylint{}): the model} cannot correctly extract data types and entities from a collection statement that spans multiple sentences. 
%\policheck{}'s NLP model is built on top of \policylint{} that constructs data and entity dependency (DED) trees as a representation of the grammatical relationships between data types, entities, and action (collect or not collect). \policheck{} can only build a complete DED tree for a complete sentence: when a collection statement consists of multiple sentences, \policheck{} produces broken DED trees for each of the sentences.
}}


%\vspace{-2pt}
%\myparagraph{\rahmadi{\policheck{} Validation.}}
\myparagraph{\minorrevision{Validation of PoliCheck results (network-to-policy consistency).}}\minorrevision{To test the correctness of PoliCheck when applied to VR apps, we \minorrevision{manually inspected all data flows from apps that provided a privacy policy,} and  checked their consistency with corresponding collection statements in the policy. Three authors had to agree on the consistency result (one of the five disclosure types) of each data flow. We found the following.}

\minorrevision{
First, we considered {\em multi-class classification} into consistent, omitted and incorrect disclosures, similar to \policheck{}'s evaluation \cite{andow2020actions}. The performance of multi-class classification can be assessed using micro-averaging or macro-averaging of metrics across classes. {\em Micro-averaging} is more appropriate for imbalanced datasets and was also used for consistency analysis of Android apps~\cite{andow2020actions} and Alexa skills~\cite{lentzsch2021heyalexa}. In our VR dataset, we obtained 84\% micro-averaged precision, recall and F1-score}\footnote{
\minorrevision{In multi-class classification, every misclassification is a false positive for one class and a false negative for other classes; thus, micro-averaged precision, recall, and F1-score are all the same (see \appdx{\appref{}~\ref{app:policheck-validation}}).
}}.
\minorrevision{This is comparable to the corresponding numbers when applying PoliCheck to mobile \cite{andow2020actions} and Alexa Skills \cite{lentzsch2021heyalexa}, which reported 90.8\% and 83.3\% (micro-averaged) precision/recall/F1-score, respectively.  For completeness, we also computed the {\em macro-averaged} precision, recall and F1-score to be 74\%, 89\%, and 81\% respectively (\appdx{see~\tabref{}~\ref{tab:policheck-eval}}).
}

\minorrevision{
Second, we considered the binary classification case (\ie{} we treat inconsistent disclosures as positive and consistent disclosures as negative samples). We obtained 77\% precision, 94\% recall, and 85\% F1-score (see \appdx{\appref{}~\ref{app:policheck-validation}} for more details). %on validation methodology and results.
%
Overall, \policheck{}, along with our improvements for \tool{}, works well on VR apps}\footnote{\minorrevision{However, the precision is lower when distinguishing between clear and vague disclosures. Our validation shows 23\% vague disclosures were actually clearly disclosed. This is because \tool{}'s privacy policy analyzer inherits the limitations of \policheck's NLP model which cannot extract data types and entities from a collection statement that spans multiple sentences.}.}.

\mycomment{
In terms of entity, first party flows account for 11.9\% (135/1,135) of data-flow tuples, and 45.2\% (61/135) of them are consistent. In contrast, among other 88.1\% (1,000/1,135) of flows (third-party and platform) only 28.8\% (289/1,001) are consistent. Apps do much worse in disclosing third-party flows than first-party flows.

Unity, accounting for 63.8\% (724/1,135) of data-flow tuples, is the prominent third-party recipient. 30.8\% (223/724) of Unity flows are consistent. Platform (\ie Oculus and Facebook) accounts for 10.7\% (122/1,135) of data-flow tuples, 27.8\% (34/122) of which are consistent. Other entities were mostly contacted by only one or two apps and accounts for only 13.6\% (154/1,135) data-flow tuples in total.

Note that the bad consistency of third-party flows does not mean that these third parties don't disclose their data collection practices. In contrast, we found Unity and Oculus privacy policies are among the most detailed and clearest ones. For example, Oculus privacy policy clearly lists the categories of information they collect (\eg \textit{Environmental, Dimensions and Movement Data}, \textit{Technical System Information}...) and specific examples of data types they refer to (\eg \textit{Technical System Information} includes \textit{user ID}, \textit{device ID} and so on). The reason for lots of omitted disclosures of these entities is that apps' privacy policies fail to cite third-party privacy policies. As discussed in \cite{andow2020actions}, developers may be not aware of their responsibility to disclosure third-party data collections, or they are not aware of how third-party SDKs in their apps collect user data.

We did another test. We tried to complement the missing third-party policy reference for all apps. To be specific, we included Oculus policies for all apps, and included Unity policies for apps using Unity SDK. Figure \ref{fig:policheck-bar-entity-alt} compares the new entity consistency result with previous result. This time, 97.1\% (703/724) of Unity flows and 95.8\% (116/122) of platform flows become consistent. This result is consistent with our observation that the Unity and Oculus privacy policies are well-written.


\subsubsection{Comparison with Android Platform}
\todo{We can claim novelty by comparing Oculus vs. mobile Android apps. For example, show the different data ontology that has nodes specific to Oculus apps.}

{\cuihao
Possible highlights:
\begin{itemize}
    \item Unity and Facebook / Oculus (the platform) dominate third-party ATS / PII flows, showing the monopoly of these entities on VR ecosystem.
    \item The VR platform hasn't been filled with advertising / tracking services.
    \item The percentage of inconsistent flows (most are omitted) is higher than Android platform. PoliCheck identified 31.1\% data flows as omitted disclosures. We have seemingly more than 50\% in VR. Possibly say VR apps have worse privacy policies.
\end{itemize}
}
}

\mycomment{
\begin{figure}[ht!]
	\centering
	\includegraphics[width=1\columnwidth]{images/plots_temp/polisis/first-party_heatmap_all_store.pdf}
	\caption{Polisis First Party (All Stores) Data Collected \vs{} Purpose}
	\label{fig:polisis-collected-fp-heatmap-all-store}
\end{figure}

\begin{figure}[ht!]
	\centering
	\includegraphics[width=1\columnwidth]{images/plots_temp/polisis/third-party_heatmap_all_store.pdf}
	\caption{Polisis  Third Party (All Stores) Data Collected \vs{} Purpose}
	\label{fig:polisis-collected-tp-heatmap-all-store}
\end{figure}
}

\mycomment{
\begin{figure*}[ht!]
	\centering
	\includegraphics[width=0.9\linewidth]{images/privacyincontext_ats.pdf}
	\caption{\textbf{Party $\rightarrow$ Data Type $\rightarrow$ Purpose $\rightarrow$ ATS.} For 150 apps in our corpus.}
	\label{fig:polisis-collected}
\end{figure*}

\begin{figure*}[ht!]
	\centering
	\includegraphics[width=0.9\linewidth]{images/privacyincontext.pdf}
	\caption{\textbf{Party $\rightarrow$ Data Type $\rightarrow$ Purpose.} For 150 apps in our corpus.}
	\label{fig:polisis-collected}
\end{figure*}

\begin{figure*}[ht!]
	\centering
	\includegraphics[width=0.9\linewidth]{images/privacyincontext_ats.pdf}
	\caption{\textbf{Party $\rightarrow$ Data Type $\rightarrow$ Purpose.} For 150 apps in our corpus.}
	\label{fig:polisis-collected}
\end{figure*}}


\begin{figure*}[t!]
	\centering
	\vspace{-10pt}
	\includegraphics[width=0.9\linewidth]{images/privacyincontext-purpose-final.pdf}
	%\vspace{-10pt}
	\caption{\textbf{Data flows in context.} We consider the data flows (\dataflowtuple) found in the network traffic, and, in particular, the 370 data flows associated with consistent disclosures. 
	%(\ie for which there are clear or vague disclosures in the privacy policy). 
	We analyze these in conjunction with their {\em purpose} as extracted from the privacy policy text \minorrevision{and depict the augmented tuples {\textit{$\langle$app, data type, destination, purpose $\rangle$}} in the above alluvial diagram. The diagram is read from left to right, for example: (1) out of 251 data flows from the Oculus app store, no more than 51 data flows collect User ID and send it to various destinations; (2) the majority of User ID is collected by Unity; and (3) Unity is responsible for the majority of data flows with the purpose of advertising. Finally, the color scheme of the edges helps keep track of the flow. From App to Data Type, the color indicates the app store: blue for Oculus apps and gray for SideQuest apps. From Data Type to Destination, the color indicates the type of data collected: PII and VR Sensory Data data flows are in orange, while Fingerprinting data flows are in green. From Destination to Purpose, we use blue to denote first-party destinations and red to denote third-party destinations.} 
	}
	\label{fig:polisis-collected}
	\vspace{-10pt}
\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Data Collection in Context}
\label{sec:polisis-context}

Consistent (\ie clear, or even vague) disclosures are desirable because they notify the user about the VR apps' data collection and sharing practices. However, they are not sufficient to determine whether the information flow is within its context or social norms.  This context includes (but is not limited to) the purpose and use, notice and consent, whether it is legally required, and other aspects of the ``transmission principle'' in the terminology of contextual integrity~\cite{privacy-in-context}. In the previous section, we have discussed the {\em consistency} of the network traffic \wrt the privacy policy statements: this provides some context. In this section, we identify an additional context: we focus on the {\em purpose} of data collection.


\myparagraph{Purpose.} 
We extract purpose from the app's privacy policy using \polisys{}~\cite{harkous2018polisis}---an online privacy policy analysis service based on deep learning. \polisys{} annotates privacy policy texts with purposes at text-segment level. We developed a translation layer to map annotated purposes from \polisys{} into consistent data flows (see \appdx{\appref{}~\ref{app:polisis-integration}}). This mapping is possible only for data flows with consistent disclosures, since we need the policy to extract the purpose of a data flow.
%We were able to the purposes of 224 (out of 1,135) data flows.
\minorrevision{We were able to process 293 (out of 359) consistent data flows}\footnote{
%For the 359 data flows, we successfully labeled 224 data flows with the purposes extracted by \polisys{}.
\minorrevision{
\polisys{} did not process the text segments that correspond to the remaining 66 consistent data flows: it did not annotate the text segments and simply reported that their texts were too short to analyze.}}
\minorrevision{ that correspond to 141 text segments annotated by \polisys{}.
Out of the 293 data flows, 69 correspond to text segments annotated as ``unspecific'', \ie  \polisys{} extracted no purpose. The remaining 224 data flows correspond to text segments annotated with purposes.
Since a data flow can be associated with multiple purposes, we expanded \minorrevision{the 224} into 370 data flows, so that each data flow has exactly one purpose.} There are nine distinct purposes identified by \polisys{} (including advertising, analytics,  personalization, legal, \etc; see \figref{}~\ref{fig:polisis-collected}).
%%
 %\todo{\hieu{what about merger and additional feature? leave it as gray area/ignore?}}

%We attempt to map the extracted data collection purposes from \polisys{} to the data flows we extracted from our network traffic dataset---recall that we have a total of \dataflowtotal{} data flows. 
%In \secref{}~\ref{sec:policheck-results}, we have reported that 359 of the \dataflowtotal{} data flows are classified as consistent disclosures---776 data flows are classified as inconsistent disclosures. 
%In other words, \polisys{} can only extract data collection purposes for the 359 data flows, each of these data flows has a correlated text segment in the app's corresponding privacy policies.
%For each data flow, \tool{}'s data-flow-to-policy analysis provides a mapping for the data flow's data type to its corresponding text segment in the privacy policy that contains the text segment.
%Thus, we can map the data flow to its originating text segment that \polisys{} extracts data collection purposes for.

\minorrevision{To further understand whether data collection is essential to app functionality, we distinguish between purposes that  support core functionality (\ie{}  basic features, security, personalization, legal purposes, and merger) and those unrelated to core functionality (\ie{} advertising, analytics, marketing, and additional features)~\cite{pii-nist-report}. 
%
Intuitively, core functionality indicates services that users expect from an app, such as reading articles from a news app or making a purchase with a shopping app.}
%
We found that only 31\% (116/370) of all data flows are related to core functionality, while 69\% (254/370) are unrelated. 
%
Interestingly, 81\% (94/116) of core-functionality-related data flows are associated with third-party entities,  indicating that app developers use cloud services.
%
\minorrevision{On the other hand, data collection purposes unrelated to core functionality can be used for marketing emails or cross-platform targeted advertisements.}
This is partly also corroborated by our ATS findings in \secref{}~\ref{sec:ats-ecosystem}: %, as many destinations are related to tracking services: 
83\% (211/254) are associated with third-party tracking entities. In OVR, data types can be collected for tracking purposes and used for ads on other mediums (\eg Facebook website) and not on the \device{} device itself.
%



%\myparagraph{Data Type Purposes}
Next, we looked into the data types exposed for different purposes. 
The majority of data flows related to core functionality (56\% or 65/116) expose PII data types, while Fingerprinting data types appear in most (66\% or 173/254) data flows unrelated to functionality. 
%
We found that 15 data types are collected for functionality: these are comprised of Fingerprinting (41\% or 48/116 data flows) and VR Sensory Data (3\% or 3/116 data flows). We found that 19 data types are collected for purposes unrelated to functionality: these are comprised of PII (26\% or 65/254 data flows) and VR Sensory Data (6\% or 16/254 data flows). Interestingly, VR Movement, VR Play Area, and VR Field of View are mainly used for ``advertising'', while VR Movement and VR Pupillary Distance are used for ``basic features'', ``security'', and ``merger'' purposes~\cite{harkous2018polisis}. 


\minorrevision{
\myparagraph{Validation of \polisys{} results (purpose extraction).} In order to validate the results pertaining to purpose extraction, \minorrevision{we read all the 141 text segments previously annotated by \polisys{}. Then, we manually annotated each text segment with one or more purposes (based on the nine distinct purposes identified by \polisys{}). We had three authors look at each segment independently and then agree upon its annotation. We then compared our annotation with the purpose output by \polisys{} for the same segment. We found that this purpose extraction has 80\%, 79\%, and 78\% micro-averaged precision, recall, and F1-score respectively\footnote{Please note that this is multi-label classification. Thus, unlike multi-class classification for \policheck{}, precision, recall, and F1-score are different.}. These micro-averaged results are directly comparable to the \polisys{}' results in \cite{harkous2018polisis}}:
\minorrevision{\tool{}'s purpose extraction works well on VR apps.}
%\athina{[AM: and are comparable or better? and why is this important?]}. 
For completeness, we also computed the macro-averaged precision, recall, and F1-score: 81\%, 78\%, and 78\%, respectively. \tabref{}~\ref{tab:polisis-eval} \appdx{in~\appref{}~\ref{app:polisis-integration}} reports the precision, recall, and F1-score for each purpose classification, and their micro- and macro-averages.} 
%\athina{[AM:Consider putting that table back in; and making that appendix more self-contained.]}



%\footnote{\rahmadi{Here, we report both the macro-averaged and micro-averaged results. In the \polisys{} paper~\cite{harkous2018polisis}, the authors reported macro-averaged results, but simply labeled them with ``Average''. In our case, we deem that micro-averaged results are more appropriate since each purpose has a different weight: support value (\ie the number of occurrences of each label in ground truth)~\cite{sklearn-support}. Further, in a multi-label classification problem; thus, unlike multi-class classification, precision, recall, and F1-score can be different.}}. 
%Thus, our results are comparable to the evaluation results for purpose annotation in the \polisys{} paper.}


%\myparagraph{Findings.}
%\figref{}~\ref{fig:polisis-collected} shows equal distribution of collected data types across apps (from both app stores). 
%As we have discussed in Section~\ref{sec:policheck-results}, data types in the PII (\eg User ID, Android ID, and Device ID) and Fingerprint (\eg Session Info, Usage Time, and SDK Version) categories are the most collected---these sensitive data flows go to first party, Unity, Oculus, and other third-party entities.
%The guidelines provided in~\cite{pii-nist-report} imply that data collection for the purposes of ``basic feature'', ``security'', ``personalization'', and ``legal'' are appropriate. 
%Even though these support the core functionality of apps, data flows attributed with these 4 purposes constitute only around 14\% (52/370) of all data flows---they are the bottom 4 of all purposes.
%Concerningly, the main purposes for data collections include advertising (32.2\% or 119/370 data flows) and analytics research (18.9\% or 70/370 data flows)---less than 10 apps in our corpus explicitly ask users to read their privacy policy or give consent to data collection (\eg for analytics purposes).



\mycomment{
82.4\% (305/370) of the data flows are third-party.
11.6\% (43/370) of the data flows are first-party.
5.9\% (22/370) of the data flows are platform-party.

776 N/A (not a vague/clear disclosure)
63 NO_MATCH (failed to find the same sentence in Polisis results) - due to different preprocessing and text segmentation and Polisis doesn't classify every sentence.
3 NO_POLISIS_OUTPUT (Polisis analysis.json doesn't exist)
69 "" (Polisis found no purpose)
224 found purposes

Total: 1,135 data flows.
}

\mycomment{
We discovered the privacy policy texts state not only that these apps collect various data types for various purposes, but also that many apps send the collected information to third parties, including more sensitive information that can be categorized as PII.
\figref{}~\ref{fig:polisis-collected-tp-heatmap-all-store} shows various data types that are sent by these apps.
Most notably, many apps send PII such as \emph{contact}, \emph{financial}, and \emph{generic personal information} to third parties.

\todo{Polisis is used to perform privacy policy text analyses. We perform textual analyses to find: (1) data types, (2) purposes. We perform a "privacy in context" analyses. Maybe we can look into (1) purposes, (2) categories, and (3) first vs. third-party as the context. Polisis also has data retention and user choice extraction.}
}

==> VR Project (USENIX Security 2022)/related_work.tex <==
%\vspace{-5pt}
\section{Related Work}
\label{sec:related-work}

%\vspace{3pt}
\paragraph{Privacy in Context.}
The framework of ``Privacy in Context"~\cite{privacy-in-context} specifies the following aspects of information flow: (1) actors: sender, recipient, subject; (2) type of information; and (3) transmission principle. The goal is to determine whether the information flow is appropriate within its context. The ``transmission principle" is key in determining the appropriateness of the flow and may  include: the purpose of data collection, notice and consent, required by law, \etc~\cite{privacy-in-context}. In this paper, we seek to provide context for the data flows (\dataflowtuple{}) found in the network traffic. We primarily focus on the network-to-policy {\em consistency}, {\em purpose} of data collection, and we briefly comment on notice and consent. Most prior work on network analysis only characterized destinations (first \vs third parties, ATS, \etc) or data types exposed without additional contexts. One exception is MobiPurpose~\cite{jin2018mobipurpose}, which  inferred data collection purposes of mobile (not VR) apps, using network traffic and app features (\eg URL paths, app metadata, domain name, \etc); the authors stated that ``the purpose interpretation can be subjective and ambiguous''. Our notion of purpose is explicitly stated in the privacy policies and/or indicated by the destination domain matching ATS blocklists.
Shvartzshnaider \etal introduced the contextual integrity (CI) framework to understand and evaluate privacy policies~\cite{shvartzshnaider2019going}---they, however, leveraged manual inspection and not automation.

% (e.g. due to insufficient or incomplete information)''. \tool{}, on the other hand, leverages \polisys{} to extract purposes directly from privacy policies written by app developers; thus, it is more objective.

%\vspace{-2pt}
%\myparagraph{Privacy of Various App Ecosystems.}
\myparagraph{\minorrevision{Privacy of various platforms.}}
The research community has looked into privacy risks in various platforms, using static or dynamic code analysis, and---most relevant to us---network traffic analysis.
Enck \etal performed static analysis of Android apps~\cite{androidappstudy} and discovered PII misuse (\eg personal/phone identifiers) and ATS activity.
Taintdroid, first introduced taint tracking for mobile apps~\cite{taintdroid}.
%Taintdroid first introduced the use of dynamic taint tracking and analysis system to track sensitive data transmission~\cite{taintdroid}.
%Alrawi \etal assessed the security aspects of IoT devices. They first systematized the existing literature to understand attack techniques, mitigations, and stakeholders. Further, they also evaluated 45 IoT devices~\cite{iotsok}. 
Ren \etal~\cite{ren2019information} did a comprehensive evaluation of information exposure on smart home IoT devices. %. They conducted large-scale experiments using 81 smart home devices set up in UK and US.
%Fernandes \etal performed static code analysis on hundreds of smart home apps and discovered \emph{overprivilege} as an issue that led to various security vulnerabilities in a smart home~\cite{iotsecurity}.
Moghaddam \etal and Varmarken \etal observed the prevalence of PII exposures and ATS activity~\cite{mohajeri2019watching,varmarken2020tv} in Smart TVs.
Lentzsch \etal~\cite{lentzsch2021heyalexa} performed a comprehensive evaluation on Alexa, a voice assistant platform.
Ren \etal~\cite{recon}, 
Razaghpanah \etal~\cite{razaghpanah2018apps}, and Shuba \etal~\cite{shuba2016antmonitor,shuba2018nomoads,shuba2020nomoats} developed tools for analysis of network traffic generated by mobile apps, and inspection for privacy exposures and ATS activity.
Our work is the first to perform network traffic analysis on the emerging \oculusvr{} platform, using dynamic analysis to capture and decrypt networking traffic on the device; this is more challenging for Unity and Unreal based apps because, unlike prior work that dealt with standard Android APIs, we had to deal with stripped binary files (\ie no symbol table). % Notably, while previous work focused on network traffic collection and analysis, \tool{} integrates both network traffic and privacy policy analyses to look into VR privacy aspects comprehensively using the framework ``Privacy in Context''.
\minorrevision{
Augmented reality (AR) is another platform the research community has been focusing on in the past decade~\cite{roesner2014security,acquisti2014face,wassom2014augmented,kotsios2015privacy,rauschnabel2018antecedents,lebeck2018towards}.
While AR augments our perception and interaction with the real world, VR replaces the real world with a virtual one.
Nevertheless, some AR privacy issues are similar to those in VR since they have similar sensors, \eg motion sensors. }

\mycomment{
\rahmadi{
\descr{Privacy of AR.}
\todo{Maybe just change this into just one sentence or something like that.}
Augmented reality (AR) is another technology, orthogonal to VR, that the research community has been looking into in the past decade.
%decade~\cite{acquisti2011faces,acquisti2011privacy,roesner2014security,acquisti2014face,wassom2014augmented,kotsios2015privacy,rauschnabel2018antecedents,lebeck2018towards}.
Roesner~\etal outlined the security and privacy concerns of AR systems~\cite{roesner2014security}.
Acquisti~\etal investigated the implications of the increasing public availability of facial images online and the rise of computer recognition capability in the context of AR 
applications~\cite{acquisti2014face}.
%applications~\cite{acquisti2011faces,acquisti2011privacy,acquisti2014face}.
Wassom~\etal explored the law, privacy, and ethical aspects of AR systems~\cite{wassom2014augmented}.
Other work studied the privacy risks of AR smart glasses~\cite{kotsios2015privacy,rauschnabel2018antecedents} and other AR devices~\cite{lebeck2018towards} from user perspectives. 
While AR augments our perception and interaction with the real world, VR replaces the real world with a virtual one.
Nevertheless, some of AR privacy issues are similar to those in VR since they have similar sensors, \eg motion sensors. 
}
}

%\vspace{-2pt}
\descr{Privacy of VR.}
Although there is work on security aspects of VR devices (\eg{} authentication and attacks on using virtual keyboards)  \cite{luooculock,8802674,duezguen2020towards,mathis2021fast},
%
%Oculock~\cite{luooculock} explored a new biometric authentication mechanism for VR platform. They looked into using human visual system (\ie eye globe movement, eyelid, extraocular muscles, cells, and surrounding nerves) as comprehensive authentication factors for VR devices. Duezguen \etal~\cite{duezguen2020towards} proposes the ZeTA protocol for secure authentication for VR.
%
the privacy of VR is currently not fully understood.
Adams \etal~\cite{adams2018ethics} interviewed VR users and developers on security and privacy concerns, and learnt that they were concerned with data collection potentially performed by VR devices (\eg{} sensors, device being always on) and that they did not trust VR manufacturers (\eg{} Facebook owning Oculus).
\minorrevision{Miller \etal present a study on the implications of the ability of VR technology to track body motions~\cite{oculus-privacy-3}.}
%In addition, developers are most concerned with causing motion sickness to the users.
%
Our work is motivated by these concerns but goes beyond user surveys to analyze data collection practices exhibited in the network traffic and stated in privacy policies. %Our tool and findings improve the transparency of data collection in VR.   
%\tool{} gives researchers a way to study \oculusvr{} in a holistic way, in terms of network traffic and privacy policy consistency. Our findings provide better transparency for the data collection practices of VR apps. 
%and computer-human interactions of VR~\cite{vr-accidents}.
% Orthogonal to VR, researchers have also looked into AR. There is a body of work that looks into the network performance of AR systems~\cite{ar-over-cellular,ar-multiuser,ar-hologram}.
%Similar to our work, they also look into the Oculus platform as the context of their study.

%\vspace{-2pt}
\descr{Privacy policy analysis.}
% From 2014 to 2021 tools have been steadlily imrpving?
Privacy policy and consistency analysis in various app ecosystems ~\cite{zimmeck2014privee,slavin2016toward,zimmeck2017automated,wang2018guileak,harkous2018polisis,andow2019policylint, andow2020actions} is becoming increasingly automated.
%This body of work has been automating privacy policy analysis by leveraging NLP and then comparing through the means of static analysis on the app's source code and dynamic analysis on the app's network traffic.
Privee~\cite{zimmeck2014privee} is a privacy policy analyzer that uses NLP  to classify the content of a website privacy policy using a set of binary questions.
Slavin \etal used static code analysis, ontologies, and information flow analysis to analyze privacy policies for mobile apps on Android~\cite{slavin2016toward}.
Wang \etal applied similar techniques to check for privacy leaks from user-entered data in GUI~\cite{wang2018guileak}.
Zimmeck \etal also leveraged static code analysis for privacy policy consistency analysis~\cite{zimmeck2017automated}; they improved on previous work by attempting to comply with legal requirements (\eg first \vs third party, negative policy statements, \etc).
%Orthogonal to this body of work, PrivacyFlashPro~\cite{zimmeck2021privacyflash} used static code analysis to generate privacy policies.
In \secref{}~\ref{sec:privacy-policy}, we leverage two state-of-the-art tools, namely  \policheck{}~\cite{andow2020actions} and \polisys{}~\cite{harkous2018polisis}, to perform data-flow-to-policy consistency analysis and to extract the data collection purpose, respectively.
\policheck{} was built on top of \policylint{}~\cite{andow2019policylint}, a privacy policy analyzer for mobile apps. It analyzes both positive and negative data collection (and sharing) statements, and detects contradictions.
%PoliCheck~\cite{andow2020actions} analyzes information flows from the network traffic to find sensitive data disclosures. It uses NLP and graph-based techniques to check whether the corresponding privacy policy has sentences that directly correspond to the sensitive data disclosures. When such sentences are not found, PoliCheck labels the app as having \emph{vague}, \emph{omitted}, \emph{incorrect}, or \emph{ambiguous} disclosure.
%Polisis~\cite{harkous2018polisis} is a framework that automatically analyzes privacy policy texts in terms of parts, purposes, \etc using NLP techniques.
Lentzsch \etal also used off-the-shelf \policheck{}  %privacy policies of Alexa skills 
 using a data ontology crafted for Alexa skills.
%In contrast, 
\tool{} focuses on \oculusvr{} and improves on \policheck{} in several ways, including VR-specific ontologies, referencing third-party policies, and extracting data collection purposes.
%Lentzsch \etal evaluated the privacy policies of Alexa skills. They used and adapted PoliCheck into this new domain to extract data flows from Alexa skills by using their permissions and perform data-flow-to-policy consistency analysis. 
%Our work, \tool{}, improves, adapts, and integrates PoliCheck and Polisis into the VR domain to perform an evaluation VR app privacy policies coupled with network traffic. 



==> additional.tex <==
\subsection{Data Minimization}
We evaluate whether the transmission of data is necessary to the functionality of an Oculus App. For that purpose, we sample a few apps based on criteria such as if they were chatty. We also randomly sample a few apps to do the following:
\begin{itemize}
    \item Offline mode: We block all network traffic to see if they are still functional. 
    \item No platform mode: We block all network traffic going to Facebook.
    \item No X system apps: We block all network traffic initiated by certain system apps. We report which system apps are important to the functionality of apps.
    \item No network traffic from app: we block all network traffic initiated by the app itself.
\end{itemize}
